Characterizing and Predicting Repeat Food Consumption Behavior for Just-in-Time Interventions

Human beings are creatures of habit. In their daily life, people tend to repeatedly consume similar types of food items over several days and occasionally switch to consuming different types of items when the consumptions become overly monotonous. However, the novel and repeat consumption behaviors have not been studied in food recommendation research. More importantly, the ability to predict daily eating habits of individuals is crucial to improve the effectiveness of food recommender systems in facilitating healthy lifestyle change. In this study, we analyze the patterns of repeat food consumptions using large-scale consumption data from a popular online fitness community called MyFitnessPal (MFP), conduct an offline evaluation of various state-of-the-art algorithms in predicting the next-day food consumption, and analyze their performance across different demographic groups and contexts. The experiment results show that algorithms incorporating the exploration-and-exploitation and temporal dynamics are more effective in the next-day recommendation task than most state-of-the-art algorithms.

==> [DPH 2019] Repeat Food Consumption/analysis.tex <==
In this section, we present a quantitative analysis of repeat food consumption behavior. Specifically, we investigate repeat consumption patterns across meal occasions, temporal lifestyle factors, and demographic groups. Firstly, let us define the notion of repeat food consumption used in the analysis. A food item by a user is considered repeated if the user has consumed the same item within the last $k$ time steps. %to be consistent with other mentioning of t,
% Explain why we don't consider the entire consumption history for repeat food consumption: 1) To ensure equal days in history for analysis for different days of the week, and for earlier dates and later dates in our records. 2) In the prediction tasks, as we use aggregated user-item consumption frequency in the training data, if entire history were used, the training sets and predictions among sessions would be marginally different. This can be especially problematic if we aim to predict the food consumption during weekends, which are shown to be dissimilar to that during weekdays as detailed below. Therefore, it is more meaningful to also restrict the data for analysis, capturing the most recent items consumed. 3) Food consumed can be forgotten if it was consumed long time ago, and become 'novel' again for a user.

Formally, let $U$ be the set of all users, $F$ be the set of all food items, and $S$ be the set of food consumption sequences of all users, $S=\{S_1, \cdots, S_{\vert U\vert} \}$. Each user $u_i \in U$ has a consumption sequence $S_i = \{X^1_i, \cdots, X^T_i\}$, where $X^t_i$ denotes the set of food items consumed by user $u_i$ at time step $t$; $X^t_i \subset F$. Next, we define the food consumption sequence of $u_i$ during the interval $[t_l,t_r)$ as  $S_{i}^{[t_l,t_r)} = \{X_{i}^{t_l}, \cdots, X_{i}^{t_r-1}\}$ and use $n_{i, j}^{t, k}=\vert\{X \in S_i^{[t, t+k)}, f_j \in X \}\vert$ to denote the number of days the food item $f_j$ is consumed by user $u_i$ during the interval $[t,t+k)$. 
% \[n_{i, j}^{t, k}=\vert\{X \in S_i^{[t, t+k)}, f_j \in X \}\vert\] 
If $n_{i,j}^{t,k} \geq 2$, $f_j$ is said to be \textit{reconsumed} by $u_i$ during the holding time window [$t$,$t+k$). 
% $n_{i,j}^{t,k}$ is called the repeat consumption count of $f_j$ by user $u_i$ in the time window.
% In this work, we consider $k$ = 7 days as the default time window.

Next, we measure the propensity to reconsume of user $u_i$ as a fraction of repeat consumptions over all consumptions of $u_i$.
% repeatedly consumed items and all items consumed. 
That is, let $\mathbb{S}^{t,k}_i = \{X \in S^{t}_i \vert  \exists f_j \in F, n_{i,j}^{t,k} \geq 2\}$ be the repeat consumptions of user $u_i$ at time step $t$, the fraction of repeat consumptions of $u_i$ at time step $t$ and the average fraction of repeat consumptions of $u_i$ given a $k$-day window size are defined in equations~\ref{eq:fraction_repeat} and~\ref{eq:average_fraction_repeat}, respectively. 

\noindent\begin{minipage}{.4\linewidth}
\begin{equation}
\label{eq:fraction_repeat}
R^{t,k}_i = \frac{\vert \mathbb{S}^{t, k}_i \vert}{\vert S^{t}_i \vert}
\end{equation}
\end{minipage}%
\begin{minipage}{.6\linewidth}
\begin{equation}
\label{eq:average_fraction_repeat}
R^{k}_i = Avg_{t \in [1,T-k+1]} R^{t,k}_i
\end{equation}
\end{minipage}

% \begin{equation}
% \label{eq:fraction_repeat}
% R^{t,k}_i = \frac{\vert \mathbb{S}^{t, k}_i \vert}{\vert S^{t}_i \vert}
% \end{equation}

% Lastly, the average fraction of repeat consumptions of $u_i$ given a $k$-day window size is defined as: 

% \begin{equation}
% \label{eq:average_fraction_repeat}
% R^{k}_i = Avg_{t \in [1,T-k)} R^{t,k}_i.
% \end{equation}

The CDF plot of the fraction of repeat consumptions ($R^{k}_i$) at different $k$-day window sizes, i.e., 2 days, 7 days, 30 days, and lifetime ($\infty$) are shown in Figure~\ref{fig:k_variation}. With smaller $k$ values, the bounded consumption sequence is shorter and the set of food items consumed by the user is generally smaller. 
% the set of food has been consumed, and thus 
% the set of food can be possibly repeated
Therefore, fewer food items can be considered 
% as ``a repeat from the past'' 
and the fraction of repeat consumptions is expected to be lowered. When $k = 7$, we observe that about 50\% of the users reconsumed the same food items up to 40\% of the time, whereas when considering past consumptions over the entire users' lifetime ($k=\infty$), about 50\% of the users reconsumed up to almost 60\% of past items. For the rest of this section, 
% we set $k = 7$ as the default time window given the human ability to recall past dietary experience ~\cite{willett1985reproducibility}.
we set $k = 7$ as the default time window given a strong recency bias towards food consumptions of the previous week.

% 6*3 inches, bbox_inches='tight', pad_inches=0.0 => size: (513, 1119)
\begin{figure}[ht]
 \includegraphics[scale=0.45,center]{figures/line_threshold.png}
 \caption{CDF of the fraction of repeat consumptions ($R^k_i$) at different $k$-day window sizes}
 \label{fig:k_variation}
\end{figure}

% Distribution of percentage repeat consumption for k variation
% \begin{tabular}{lrrrr}
% \toprule
% {} &       k=2 &       k=7 &      k=30 &     k=inf \\
% \midrule
% count &  7721.000 &  7721.000 &  7721.000 &  7721.000 \\
% mean  &     0.229 &     0.395 &     0.488 &     0.560 \\
% std   &     0.122 &     0.164 &     0.179 &     0.189 \\
% min   &     0.000 &     0.000 &     0.000 &     0.000 \\
% 25\%   &     0.139 &     0.279 &     0.365 &     0.432 \\
% 50\%   &     0.216 &     0.396 &     0.500 &     0.574 \\
% 75\%   &     0.305 &     0.511 &     0.619 &     0.704 \\
% max   &     0.820 &     0.916 &     0.948 &     0.979 \\
% \bottomrule
% \end{tabular}

\subsection{Meal Occasions and Carryover Effects}
\label{sec:meal_occassions}
Next, we investigate the presence of \textit{carryover} effects -- the influence of past food consumption behavior on current food consumption behavior \cite{Khare2006}, and the repeat consumption patterns in different meal occasions, i.e., breakfast, lunch, dinner, and snack, in our dataset. Specifically, we aim to characterize the repeat consumption behavior within the same meal occasions (e.g., breakfast $\rightarrow$ breakfast) and across different meal occasions (e.g., breakfast $\rightarrow$ lunch).
First, we define the fraction of \textit{within-meal} repeat consumptions $R^{m,k}_i$ of user $u_i$ in a similar manner as the fraction of repeat consumptions $R^k_i$ (equation~\ref{eq:average_fraction_repeat}). Let $X^{b,t}_i$, $X^{l,t}_i$, $X^{d,t}_i$ and $X^{s,t}_i$ denote the subsets of items consumed by user $u_i$ at time step $t$ in four different meal occasions: breakfast, lunch, dinner, and snacks, respectively, we computed $R^{m,k}_i$ from $X^{b,t}_i$, $X^{l,t}_i$, $X^{d,t}_i$ and $X^{s,t}_i$ for the corresponding meal occasions.
According to the CDF plot of fraction of within-meal repeat consumptions in Figure~\ref{fig:repeat_perc_meal}, breakfast has the highest within-meal fraction of repeat consumptions ($R^{m,k}_i$) amongst all meal occasions. That is, about 50\% of users reconsumed up to 50\% of the past breakfast items in the last 7 days. On the other hand, dinner has the lowest $R^{m,k}_i$, where 50\% of users only reconsumed up to 17\% of the past dinner items.

\label{sec:meals}
% 6*3 inches, bbox_inches='tight', pad_inches=0.0 => size: (513, 1119)
\begin{figure}[thp]
 \includegraphics[scale=0.45,center]{figures/line_meal.png}
 \caption{CDF of fraction of within-meal repeat consumptions ($R^{m,k}$) of 4 different meal occasions}
 \label{fig:repeat_perc_meal}
\end{figure}

% heatmap using vmax=.4, vmin=.05,
% 5*4.5 inches, bbox_inches='tight', pad_inches=0.0 => size: (786, 905)
\begin{figure}[thp]
\includegraphics[scale=0.45,center]{figures/heatmap_meal.png}
\caption{Fractions of within-meal ($R^{m,k}$) and across-meal ($R^{m,m',k}$) repeat consumptions, averaged across all users}
\label{fig:heatmap_meal}
\end{figure}
% Heatmap data, p for preceding
% Current &  breakfast &  dinner &  lunch &  snack \\
% p\_breakfast &       0.48 &    0.04 &   0.05 &   0.07 \\
% p\_dinner    &       0.05 &    0.20 &   0.11 &   0.04 \\
% p\_lunch     &       0.07 &    0.07 &   0.27 &   0.06 \\
% p\_snack     &       0.08 &    0.03 &   0.05 &   0.32 \\

% Heatmap data distribution
% mean      0.12
% std       0.13
% min       0.03
% 25%       0.05
% 50%       0.07
% 75%       0.13
% max       0.48

% \begin{tabular}{lrrrr}
% meal\_index &  perc\_breakfast &   perc\_lunch &  perc\_dinner &   perc\_snack \\
% count &     6827.000000 &  6879.000000 &  6808.000000 &  7647.000000 \\
% mean  &        0.477141 &     0.262255 &     0.198613 &     0.310324 \\
% std   &        0.230747 &     0.189535 &     0.163913 &     0.200675 \\
% min   &        0.000000 &     0.000000 &     0.000000 &     0.000000 \\
% 25\%   &        0.307692 &     0.119048 &     0.074262 &     0.157895 \\
% 50\%   &        0.488889 &     0.232558 &     0.167509 &     0.297872 \\
% 75\%   &        0.650000 &     0.375000 &     0.291667 &     0.447434 \\
% max   &        0.992366 &     0.971237 &     0.931419 &     0.993410 \\
% \caption{Data summary for figure 6}
% \end{tabular}

Next, we define the fraction of \textit{across-meal} repeat consumptions $R^{m, m',k}_i$ of user $u_i$ for meal $m$ with respect to the past consumptions in the holding time window of meal $m'$; $m \neq m'$. 
% This is because when $m \eqn m^\prime$, $R^{m, m^\prime,k}_i$ is equivalent to $R^{m,k}_i$ and refers to within-meal.
Then, we computed $R^{m,m',k}_i$ for the twelve corresponding meal occasion pairs for all users. Figure~\ref{fig:heatmap_meal} displays the fractions of within-meal ($R^{m,k}$ in the diagonal cells) and across-meal ($R^{m,m',k}$ in the non-diagonal cells) repeat consumptions, averaged across all users. As we can see, the across-meal carryover effects are much weaker than the within-meal carryover effects.
% The strongest across-meal carryover effect is found between the preceding dinner and the current lunch (dinner $\rightarrow$ lunch); $R^{m,m',k}$ = 0.111 (S.D. = 0.118). This is within our expectation as the food items consumed at lunch and dinner are generally more similar and interchangeable than other meals.
The strongest across-meal carryover effect is found between the preceding lunch and the current dinner (lunch $\rightarrow$ dinner); $R^{m,m',k}$ = 0.111 (S.D. = 0.118). This is within our expectation as the food items consumed at lunch and dinner are generally more similar and interchangeable than other meals. It is rather common to eat lunch leftover at dinner.
    %   	breakfast 	dinner 	lunch 	snack
% p_breakfast 	0.481 	0.037 	0.054 	0.070
% p_dinner 	0.052 	0.205 	0.111 	0.040
% p_lunch 	0.068 	0.075 	0.265 	0.057
% p_snack 	0.079 	0.032 	0.052 	0.319
% The differences in magnitude between within-meal and across-meal are also greater at breakfast than at snack, dinner, and lunch.
These findings are also in line with prior consumer research \cite{Khare2006}.

% % similar results if we do not do the filtering by the complete 4 preceding records
% Next, we study the carryover effects in terms of food types among meals. Carryover habit obtains when the food types consumed in preceding meals influence their consumption in the current meal. We look at the distributional differences of 66 food subcategories for a user's food choices in a meal and the preceding breakfast, lunch, dinner and snack. 
% % We first calculate the normalized frequencies of all 66 food categories for each meal, which has a complete records of the 4 preceding meals (316,651 records, or 27.5\% of all meal records). 
% For each meal record of a user, we identify the food consumed by the user in the immediate preceding meal of all four meal occasions. For instance, for $X^{l,t}_i$, the lunch record of user $u_i$ at time step $t$, the immediate preceding meals are $\mathbb{X}^{l,t}_i = {X^{b,t}_i, X^{l,t-1}_i, X^{d,t-1}_i, X^{s,t-1}_i}$. The immediate preceding meal records are defined for each meal record of breakfast, dinner and snack in similar manners. 
% % Another example is for $X^{s,t}_i$, the snack record of user $u_i$ at time step $t$, the immediate preceding meals are $X^{b,t}_i$, $X^{l,t}_i$, $X^{d,t}_i$ and $X^{s,t-1}_i$.
% For our analysis, we only focus on the meal records with all immediate preceding meals containing at least some food items (i.e. the user did not skip recording the meal). 
% % Thus we have 316,651 meal records, or 27.5\% of all meal records.
% % Or: focus on the meal records with some immediate preceding meals containing at least some food items (i.e. the user did not skip recording the meal). - the results will be similar
% Then we calculate the Jensen-Shannon distance between the consumption distribution of a meal and those of the four preceding meals. A small distance indicates that the food consumption patterns between the two meals are compositionally similar.
% Figure~\ref{fig:heatmap_meal} indicates a meal is more similar to the preceding same meal, rather than immediate prior meals. That is, the within-meal carryover effect is the stronger than the between meal carryover effects \cite{Khare2006}. 
% % H2 of Habitual Behavior in American Eating Patterns: The Role of Meal Occasions
% The strongest cross-meal carryover effect occurs between the preceding lunch and the current dinner. This is within out expectation as the diet for lunch and dinner are generally more similar and interchangeable. 
% In addition, we find out that breakfast, compared to any other meal, is more influenced by preceding meals \cite{Khare2006}. 
% % H1 also met: The magnitude of carryover habit will be stronger at breakfast than at lunch and dinner.
% % b    0.511975 
% % l    0.545584
% % d    0.575396
% % s    0.552435
% The difference between within-meal and across-meal is also greater at breakfast than at lunch, dinner and snack \cite{Khare2006}.
% % H3 also met: The difference in magnitude between within-meal carryover habit and across-meal carryover habit will be greater at breakfast than at lunch and dinner.
% % b    0.309717
% % l    0.144096
% % d    0.107935
% % s    0.220180

\subsection{Temporal Dynamics of Consumption}
\label{sec:temporal}
% 6*3 inches, bbox_inches='tight', pad_inches=0.05 => size: (544, 1143)
\begin{figure}[thp]
 \includegraphics[scale=0.45,center]{figures/ts_perc_repeat.png}
 \caption{Fraction of daily repeat consumptions ($R^{t,k}$) over time}
 \label{fig:repeat_trends}
\end{figure}

% 6*3 inches, bbox_inches='tight', pad_inches=0.2 => size: (794, 910)
\begin{figure}[thp]
 \includegraphics[scale=0.45,center]{figures/box_weekday.png}
 \caption{Distribution of fraction of daily repeat consumptions ($R^{t,k}$) for days of the week}
 \label{fig:box_weekday}
\end{figure}

Furthermore, we explore the impact of temporal lifestyle factors, such as the weekday-weekend cycle, on the repeat consumption behavior over the 6-month period. At each time step $t$, we computed the fraction of \textit{daily} repeat consumptions across all users as $R^{t,k} = Avg_{u_i \in U} R^{t,k}_i$ where $t$ represents day of the year. As shown in Figure~\ref{fig:repeat_trends}, there is a clear cyclical and habitual pattern in the repeat consumption behavior where the fractions of daily repeat consumptions fluctuate in a weekly cycle yet the trend remains more or less constant over a long period of time. The fractions of daily repeat consumptions are greatly lower during the Thanksgiving and the Christmas holidays in the US, possibly due to temporary changes to seasonal food choices. 
% These patterns are consistent with the finding shown in Figure~\ref{fig:heatmap_behavior}\protect\subref{fig:heat_weeks}. 
The day with the lowest fraction of daily repeat consumption is the first Monday of 2015 ($R^{t,k}$ = 0.379), largely due to the surge in newly active users, whose past consumption data were far fewer than the users in the preceding periods.
% The history may > 7,  but probably the consumption record happens very early. In other words, the 1st Monday in 2015 is a start of a new lifetime for the newly active user.
Next, Figure~\ref{fig:box_weekday} displays the distribution of $R^{t,k}$ for different days of the week. As shown here, the medians and the variability of $R^{t,k}$ for all weekdays are higher than those of weekends, suggesting that the users were more likely to engage in variety-seeking behavior during the weekends than the weekdays. Within the weekdays, the fractions of repeat consumptions are the lowest on Monday and continue to rise as the week progresses until reaching the peak on Thursday. This may also indicate the presence of carryover effects as the users' daily eating habits were picked up from one weekday to the next. 
% Similarly, these patterns are in accordance with the previous finding shown in Figure~\ref{fig:heatmap_behavior}\protect\subref{fig:heat_weekdays}.

% Next, we zoom into the details between distributions of fractions of repeat consumption between days of the week with a box plot. As indicated in Figure~\ref{fig:box_weekday}, weekends have similar centres, which are lower than those of weekdays, suggesting that users tend to explore more food choices on weekends. We also find out that weekends have smaller variability than weekdays. Among weekdays, Mondays and Fridays have lower centers and smaller variability than Tuesdays, Wednesdays and Thursdays. The distribution of the repeat consumption percentage on Mondays and Fridays are skewed to the left, while Tuesdays, Wednesdays and Thursdays are reasonably symmetric.

% Interconsumption interval analysis can be found in /backup/ici.tex
%\input{backup/ici.tex}
\subsection{Demographic Differences}
Does the propensity to reconsume differ significantly between demographic groups? In this section, we compare the repeat consumption behaviors of users in the following subgroups based on their demographic attributes: genders (female and male users), age groups (younger adults aged 18-44 years old and older adults aged 45 years and older), and regions of residence in the US including northeast (NE), midwest (MW), south (S), and west (W). For each user $u_i$, we computed the fraction of repeat consumptions $R^{k}_i$ and averaged all values of $R^{k}_i$ across all users belonging to the same demographic subgroups to get the fraction of aggregated repeat consumptions $R^{d,k}$ for the subgroups. To measure the differences of $R^{d,k}$ between the demographic subgroups, we performed Kruskal-Wallis H test with Dunn's multiple comparison test at the significance levels of 0.01 and 0.05. According to Figure~\ref{fig:demographic_repeat}, male users, older adults, and those in the northeast generally had a higher propensity to reconsume than their counterparts. Specifically, males had a significantly higher $R^{d,k}$ than females (p\textless 0.01), whereas older adults had a significantly higher $R^{d,k}$ than younger adults (p\textless 0.01). Next, there was a significant difference between $R^{d,k}$ of users in different regions (p\textless 0.05), specifically, users in the northeast had a significantly higher $R^{d,k}$ than those in the south (p\textless 0.05).

\label{sec:demo_dff}
% 6*3 inches, bbox_inches='tight', pad_inches=0.0 => size: (517, 1115)
\begin{figure}[thp]
 \includegraphics[scale=0.45,center]{figures/demographic.png}
 \caption{Fraction of aggregated repeat consumptions of different demographic groups. The groups with the highest mean are highlighted in darker color.}
 \label{fig:demographic_repeat}
\end{figure}

Compared to previous research, our finding about the age differences is in line with prior knowledge about differences in sensation seeking traits \cite{Roberti2004} in which younger people are more likely to seek out novel and varied sensations and experiences than older people. However, our finding about the gender differences is in contrary to previous findings. Specifically, male users in our study had a significantly lower tendency for novel consumptions than female users, whereas male adults generally score higher in sensation seeking traits than females \cite{Roberti2004}. One possible reason could be due to the potential interaction effect between gender and age since the average age of the male users in our study (39.5 years; S.D. = 10.7) is much higher than that of the female users (35.4 years; S.D. = 10). Lastly, to our knowledge, this study was the first to report the inter-regional differences in repeat consumption tendencies.

% Summary paragraph here
\textbf{Summary of Findings}: According to the quantitative analysis, repeat food consumption patterns displayed a recency bias. The majority of users repeatedly consumed at least 50\% of food items recently consumed within the last 7 days, whereas the repeat consumption rate went up to 60\% or higher once the entire consumption history (up to six months) was considered.
% For more than half of the users, 20\% of the food choices were the same as the food consumed in the previous day, 40\% are same as those in the previous week, 50\% are same as those in the previous month.
Furthermore, the individuals' repeat consumption tendencies significantly differed across meal occasions, temporal lifestyle factors, and demographic groups. First, there were greater patterns of the within-meal carryover effect than the between-meal carryover effect. In particular, users tended to reconsume more during breakfast and snack. However, they tended to explore novel food choices more frequently during lunch and dinner.
% explored more food options during dinner and lunch, and exploited previous food choices more in breakfasts and snacks. In addition, we identified that across-meal repeat consumption was low and food items are meal occasion specific.
Next, the repeat consumption behavior clearly exhibited a weekday-weekend. That is, users were significantly more likely to engage in variety-seeking behavior in food consumption during the weekends (and holidays) than the weekdays. 
% For the impact of temporal lifestyle factors, we identified a clear and consistent weekday-weekend cycle on the repeat consumption behavior, whereas users were more likely to engage in variety-seeking behavior during the weekends than the weekdays. 
% In addition, for special occasions, such as during the Thanksgiving and the Christmas holidays, repeat consumption was lower, possibly due to temporary changes to seasonal food choices. 
Furthermore, we observed a significantly higher repeat consumption tendency amongst male users, older adults, and users residing in the northeast of the United States, compared to their respective counterparts.
% For demographic groups, we identified that older adults had a significantly higher repeat consumption than younger adults. In addition, male users and residence in the Northeast of US in our study had a significantly lower tendency for novel consumptions than female users, and residence of other US regions.

% For regional effects, may be this is relevant: https://pubag.nal.usda.gov/download/34134/PDF - South is not significant, West and Midwest is significant for predicting Purchase Variety Across Grocery Categories based on Simpson and CS75 (probit). More are significant for cereal brands.

% Psychological studies suggest experience seeking declines with age \cite{Roberti2004}. This means that the younger adults are expected to have higher tendency for variety and less repeat consumption. This aligns with our findings. However, in terms of gender, men are consistently more sensation seeking than women\cite{Roberti2004}. Female users are thus expected to have more repeat consumption than male users. However, the MFP food diary records suggest that males are significantly more likely to repeat food choices than females, which contradict the self-reported psychological studies. This could be due to the interaction effects between gender and age, as in our studies, male users have an age mean of 39.5 (S.D. = 10.7), much higher than that of female users (35.4, S.D. = 10.0). 
% In addition, previous studies mainly rely on the self-reported questionnaires in previous, which may be less reliable compared with true consumption data.
% There are no prior results for regions of residence.
% Users the northeast regions, although younger in age on average, have more tendency of repeat consumption.

% Age mean by gender
% Female    35.440260 +- 10.016690
% Male      39.505963 +- 10.679132
% Age mean by US regions
% Northeast    35.6 +- 10.2
% Midwest      37.2 +- 10.1
% South        36.8 +- 9.9
% West         36.5 +- 10.4

% sensation seeking - Experience Seeking
% Sensation seeking is a preference to seek out varied, novel, and complex sensations and experience. Variation in food consumption is an attractive source of stimulation for sensations seekers. In Zuckerman's Sensation Seeking Scale, version V (SSS-V) questionnaire, trying new food is a key item in evaluating one's propensity of experience seeking, or the interest in low-risk, novel experiences, which is an aspect of sensation seeking\cite{Zuckerman1978}. Past studies have shown that in terms of experience seeking, females score higher than males\cite{Roberti2004}. This aligns with in our study, as MFP food diary records suggest that females are significantly less likely to repeat their food choices than females. On the other hand, experience seeking declines with age\cite{Roberti2004}. In our study, older adults are significantly less likely to repeat their food choices than younger adults. There are no prior results for regions of residence.
% sensation seeking - Boredom Susceptibility
% Our results differ from the psychological literature of sensation seeking. Past research has shown that in terms of boredom susceptibility, men are consistently more sensation seeking than women based on self-reported questionnaires\cite{Roberti2004, Cross2013}. This means that the male users dislike repetition — for example, the same food too many times in a row. However, the MFP food diary records suggest that males are significantly more likely to repeat their food choices than females, which contradict the self-reported psychological study. On the other hand, in terms of age, psychological studies suggest that boredom susceptibility is consistent across age.

% others:
% case study, most \& least repeated users
% user consistency along the timeline in terms of repeat consumption 
% food healthiness: by is_fast_food tag; by energy-dense, nutrient-poor (EDNP) classification (different criteria exist for food and beverage)
% frequency threshold - no longer presented 
% In this subsection, we would like to select a frequency threshold while keeping the holding time window size to be 7 days.
%If an item $f_i$ is consumed by a user $u_i$ in no less than $k$ meals, $m_i$ is considered to be repeatedly consumed by user $u$. 
% Let $M_i$ denote the set of meals consumed by user $u_i$. $M^b_i$, $M^l_i$ and $M^d_i$ denote the set of meals which are breakfast, lunch and dinner respectively. Let $F^r_i(k)$ denote the set of repeatedly consumed food items by $u_i$ with \textbf{repeat consumption threshold} $k$ ($k \geq 2$). As $k$ increases, the repeatedly consumed food items become ones that are more favored by $u_i$. We should expect that food items with high repeat consumption threshold should appear in more daily entries of $u_i$ than those with low repeat consumption threshold. 

==> [DPH 2019] Repeat Food Consumption/context_aware_results.tex <==
% \subsection{Context-Aware Evaluation}
% Figure~\ref{fig:ndcg} displays nDCG@5 of the best algorithm, i.e., \textbf{MixtureTW}, for different \protect\subref{fig:gender_ndcg} genders, \protect\subref{fig:age_ndcg} age groups, \protect\subref{fig:region_ndcg} regions of residence, \protect\subref{fig:day_ndcg} days of the week, \protect\subref{fig:weekday_ndcg} weekdays and weekends, and \protect\subref{fig:meal_ndcg} meal occasions. 
Do diverse groups of users equally receive the same benefits from the recommendations generated by the best algorithm, i.e., \textbf{MixtureTW}? Figure~\ref{fig:ndcg} displays nDCG@5 of \textbf{MixtureTW} for different genders, age groups, regions of residence, days of the week, weekdays and weekends, and meal occasions.
The best result is highlighted in a darker shade for each group. As we can see, there is a clear bias between the algorithm performance and the propensity to reconsume of the users in different contexts and demographic groups, previously presented in sections \ref{sec:analysis}. 
% Mainly, \textbf{MixtureTW} was more effective in predicting daily food consumption patterns of the users in the demographic groups with higher average fraction of repeat consumptions as described in section \ref{sec:analysis}. 
% In contrast, the best latent-factor model based algorithm, i.e., NMF, was more effective at predicting the daily food consumption patterns of those with lower average fraction of repeat consumptions. The performance of different algorithms was more consistent when predicting daily food consumption patterns of the users in different temporal factors and meal occasions. That is, all algorithms were more effective in the eating contexts in which the users had a higher propensity to reconsume, e.g., weekdays and breakfast.

\begin{figure}[htp]
\centering
\begin{subfigure}{0.3\columnwidth}
    \includegraphics[width=\textwidth]{figures/result_highlighted_Gender.png}
    \caption{Genders}
    \label{fig:gender_ndcg} 
\end{subfigure}
\hfill
\begin{subfigure}{0.3\columnwidth}
    \includegraphics[width=\textwidth]{figures/result_highlighted_Age_Groups.png}
    \caption{Age groups}
    \label{fig:age_ndcg}
\end{subfigure} 
\hfill
\begin{subfigure}{0.3\columnwidth} 
    \includegraphics[width=\textwidth]{figures/result_highlighted_US_Regions.png}
    \caption{Regions}
    \label{fig:region_ndcg}
\end{subfigure}  \\
% 
\begin{subfigure}{0.3\columnwidth} 
    \includegraphics[width=\textwidth]{figures/result_highlighted_day.png}
    \caption{Days of the week} 
    \label{fig:day_ndcg}
\end{subfigure} 
\hfill
\begin{subfigure}{0.3\columnwidth} 
    \includegraphics[width=\textwidth]{figures/result_highlighted_weekday.png}
    \caption{Weekdays} 
    \label{fig:weekday_ndcg} 
\end{subfigure} 
\hfill
\begin{subfigure}{0.3\columnwidth} 
    \includegraphics[width=\textwidth]{figures/result_highlighted_Meal.png}
    \caption{Meal occasions} 
    \label{fig:meal_ndcg}
\end{subfigure}
\caption{MixtureTW's performance for different demographic groups and contexts. The groups with the highest nDCG@5 are highlighted.}
\label{fig:ndcg}
\end{figure}

For different genders and age groups, the differences in the nDCG@5 were significant across all between-group comparisons (p \textless 0.01). Overall, \textbf{MixtureTW} was able to predict the daily eating habits of males 9.03\% better than females. 
The average nDCG@5 for males is 0.459 (S.D. = 0.195), whereas the average nDCG@5 for females is 0.421 (S.D. = 0.195). 
% Males can be  better predicted 9.03\% than females in terms of nDCG@5. 
% Not sure what to write for more details, 0.459/0.421-1 = 9.03\% 
Next, \textbf{MixtureTW} was 8.81\% more effective in predicting the food consumptions of older users than younger users. 
The average nDCG@5 is for users at least 45 years old is 0.457 (S.D. = 0.199), whereas the average nDCG@5 for users between 18 and 44 is 0.420 (S.D. = 0.194). 
% Older users can be 8.81\% better predicted than females in terms of nDCG@5.
Moreover, there were no significant differences between the nDCG@5 of the users in different regions of residence. 
% The highest  average nDCG@5 is for the users from the Northeast (S.D. = 0.198), which is 4.65\% higher than the lowest nDCG@5 group, i.e., the Midwest; nDCG@5 = 0.409 (S.D. = 0.198).

In terms of temporal lifestyle factors, there was a significant difference in the nDCG@5 between weekdays and weekends (p \textless 0.01). That is, \textbf{MixtureTW} was 17.15\% more effective in predicting food consumption during weekdays than weekends. The average nDCG@5 for weekdays is 0.485 (S.D. = 0.021), whereas the average nDCG@5 for weekdays is 0.414 (S.D. = 0.017). 
Next, there was a significant difference in the nDCG@5 of different days of the week (p \textless 0.01). 
Specifically, the differences were significant (p \textless 0.01) for all weekday-weekend pairs (except for Monday-Sunday being significant with p \textless 0.05). Amongst the weekday pairs, Monday had a significantly lower nDCG@5 than Wednesday (p \textless 0.01) and Thursday (p \textless 0.05). However, there were no significant differences between the nDCG@5 for the other weekday pairs (e.g., Monday vs. Tuesday) and the weekend pair (Saturday vs. Sunday). 
Wednesdays had the highest nDCG@5 (mean = 0.498; S.D. = 0.011), which is 21.76\% higher than that of the lowest group, i.e., Saturdays; nDCG@5 = 0.409 (S.D. = 0.019).

Lastly, there was a significant difference between the nDCG@5 of different meal occasions (p \textless 0.01). Furthermore, the differences in the nDCG@5 across all meal pairs were also significant (p \textless 0.01). 
Specifically, \textbf{MixtureTW} was significantly more effective in predicting food consumptions during breakfast (nDCG@5 = 0.563; S.D. = 0.250) than the other meals. On the other hand, dinner was the most challenging meal to predict (nDCG@5 = 0.217; S.D. = 0.188). The performance gap between breakfast and dinner is 159.45\%, the highest amongst any between-group differences.

% Summary paragraph here
\textbf{Summary of Findings}: We observed significant algorithmic bias in the context-aware evaluation of \textbf{MixtureTW}. Overall, \textbf{MixtureTW} was more effective in predicting daily food consumption patterns of the users in the meal occasions, temporal lifestyle factors, and demographic groups with higher average fraction of repeat consumptions as shown in sections \ref{sec:meal_occassions}, \ref{sec:temporal}, and \ref{sec:demo_dff}, respectively.
% As shown above, males, users of 45 years and above, weekdays, and breakfasts are significantly better predicted by \textbf{MixtureTW}. Thus, the model performed consistently better for user groups and eating contexts with higher repeat consumption. 
% Thus, the model was biased toward the user groups and eating contexts with higher repeat consumption. 
Specifically, male and older-adult users unevenly received greater benefits from \textbf{MixtureTW}'s recommendations than their counterparts. Interestingly, although there was a significant difference in the repeat consumption tendency amongst different regions (shown in section \ref{sec:demo_dff}), there was no algorithmic bias across regions.

% The outcomes of the context-aware evaluation provide important implications for the effectiveness of food recommender systems in the just-in-time healthy eating interventions. 
% First, as previously shown, the performance of the best algorithms was biased toward specific demographic groups and eating contexts. Thus, future food recommendation research should focus on improving the prediction accuracy of the underserved groups. More importantly, the best algorithms were not able to effectively predict the daily eating habits of certain demographic groups, who are high-priority targets of behavioral interventions due to their low tendency to adopt healthy eating behaviors \cite{Achananuparp2018}, such as young adults. Similarly, the food consumption patterns in certain eating contexts, where the users are more likely to make unhealthy food choices (e.g., weekends and dinners), were relatively more difficult to predict by the best algorithms. Therefore, food recommender systems should take into account the healthy eating behaviors of the affected groups and contexts when addressing the challenge of algorithmic bias.

% Liu Yue's old writing
% As discussed earlier, repeat consumption tendency is different across demographic groups, temporal lifestyle factors, and meal occasions. We also investigate how the model performs in the prediction tasks under the specific contexts. 

% We take a look at the prediction performance of each model toward users of different demographic groups, since we have found that the repeat consumption tendency varies among them. We select nDCG@5 as the evaluation measure. Since the evaluation is on the user level, we compute the users prediction accuracy as the average prediction accuracy of the users over all sessions. 
% $Avg_{t \in T} nDCG@m(i)_t$. 
% In addition, to measure the differences of the average nDCG@5 
% $Avg_{t \in T} nDCG@m(i)_t$ 
% between the demographic groups and contexts, we performed Kruskal-Wallis H test with Dunn's multiple comparison test at the significance level of 0.01 and 0.05.


% old figure, spanning 2 columns
% \begin{figure*}[th]
% % \centering
% \scalebox{0.8}{
% \begin{tabular}{ccc}
% \subfloat[Genders]{\includegraphics[scale=0.48]{figures/result_highlighted_Gender.png}\label{fig:gender_ndcg}} &
% \subfloat[Age groups]{\includegraphics[scale=0.48]{figures/result_highlighted_Age_Groups.png}\label{fig:age_ndcg}} &
% \subfloat[Regions of residence]{\includegraphics[scale=0.48]{figures/result_highlighted_US_Regions.png}\label{fig:region_ndcg}} \\
% \subfloat[Days of the week]{\includegraphics[scale=0.48]{figures/result_highlighted_day.png}\label{fig:day_ndcg}} &
% \subfloat[Weekdays and weekends]{\includegraphics[scale=0.48]{figures/result_highlighted_weekday.png}\label{fig:weekday_ndcg}} &
% \subfloat[Meal occasions]{\includegraphics[scale=0.48]{figures/result_highlighted_Meal.png}\label{fig:meal_ndcg}}
% \end{tabular}
% }%end scalebox
% \caption{Algorithm performance for different demographic groups and contexts. The groups with the highest nDCG@5 are highlighted.}
% \label{fig:ndcg}
% \end{figure*}

% \textbf{Gender}: 
% Among all the models, Personal and Mixture, which performs the best for the general populace as we have discussed preciously, males have a significantly higher user prediction accuracy than females (p\textless 0.01) as shown in Figure~\ref{fig:ndcg}\protect\subref{fig:gender_ndcg}.
% % This may be due to the fact that the two models rely heavily on the food consumption of the same user. Male users, with tendency to repeatedly consume as indicated in previous section, will thus be more accurately predicted for their food choices. 
% On the other hand, for NMF
% % and all other algorithms which has little or no reliance on users' own consumption patterns
% , females have a significantly higher user prediction accuracy than females (p\textless 0.01).

% \textbf{Age groups}: 
% Figure~\ref{fig:ndcg}\protect\subref{fig:age_ndcg} indicates that for all models, regardless of the overall performance of the algorithm, older adults have a significantly higher user prediction accuracy than younger adults (p\textless 0.01).

% \textbf{Regions of residence}: 
% Next, for Mixture and Personal, there is no significant difference in terms of prediction accuracy of users in different regions at the significance level of 0.05, although the mean of user prediction accuracy for Northeast is the highest among the four regions, as shown in Figure~\ref{fig:ndcg}\protect\subref{fig:region_ndcg}.
% For NMF model, there is a significant difference in terms of prediction accuracy of users in different regions (p\textless 0.01). Specifically, users in the west and northeast have significantly higher user prediction accuracy than those in the midwest and south, users in the midwest higher than those in the south (p\textless 0.05).
% nmf_model
% 5.465042888314225e-12
% order = ['Northeast', 'Midwest', 'South', 'West']
% true median = 0.22 0.20 0.18 0.24
% ('Northeast', array([ True,  True, False])) => (NE vs M), (NE vs S)
% ('Midwest', array([0.04321952, 0.0011746 ]))
% ('Midwest', array([ True,  True])) => (MW vs S), (MW vs W)
% ('South', array([6.12735898e-10]))
% ('South', array([ True])) => (S vs W)


% Next, take a look at the prediction accuracy, $nDCG@m$ at different sessions, of each model for different days of the week, and between weekdays and weekends.

% \textbf{Day of the week}:
% % Abbreviation: Monday(M), Tuesday(T), Wednesday(W), Thursday(TH), Friday(F), Saturday(SA), Sunday(SU). 
% Figure~\ref{fig:ndcg}\protect\subref{fig:day_ndcg} displays the nDCG@5 of different days of the week. For Mixture and Personal, there is a significant difference in $nDCG@m$ of different days in the week (p\textless 0.01). Specifically, weekends have significantly lower $nDCG@m$ than weekdays (p\textless 0.05).
% % Wednesdays have the highest mean $nDCG@m$, whereas Saturdays have the lowest mean $nDCG@m$, 
% For NMF, there is a significant difference in $nDCG@m$ of different days in the week (p\textless 0.01). Specifically, 
% Fridays have significantly lower $nDCG@m$ than Mondays and Tuesdays,
% Saturdays have significantly lower $nDCG@m$ than Mondays to Thursdays,
% Sundays have significantly lower $nDCG@m$ than Tuesdays (p\textless 0.05).
% % Tuesdays have the highest mean $nDCG@m$, whereas Saturdays have the lowest mean $nDCG@m$, 
% % NMF: (Mon>Fri), (Tue>Fri), (Mon>Sat), (Tue>Sat), (Wed>Sat), (Thur>Sat), (Tue >Sun), 

% \textbf{Weekdays vs weekends}:
% % Abbreviation: Weekdays(Wkday), Weekends(Wknd). 
% Figure~\ref{fig:ndcg}\protect\subref{fig:weekday_ndcg} indicates that for all models, weekdays have a significantly higher $nDCG@m$ than weekends (p\textless 0.01).

% Finally, we also investigate how the model performs in the prediction of specific meals. The set-up for next-meal prediction slightly differ from the next-day food prediction. This is because we have found that only the same type of meal in important in determining the food choices in a next meal. Therefore, the train, validate and test data are limited to the food consumption records of a specific meal for each session. Due to space constraint, we will not present the data summary and the results for next-meal prediction.

% \textbf{Meals}: 
% Abbreviation: breakfast(B), lunch(L), dinner(D), snack(S). Next-day prediction(Day) is also included as a reference.
% All Combination(4,2) pairs are significant for Dunn's test for all algorithms.
% Figure~\ref{fig:meal_ndcg} indicates that for all models, there is a significant difference in $nDCG@m$ of different meal occasions (p\textless 0.01). Specifically, breakfasts have the largest $nDCG@m$, followed by snacks, lunches and dinners (p\textless 0.01). 
% More over, compared with next-day set-up (Day), breakfasts have higher $nDCG@m$, snacks, lunches and dinners have lower $nDCG@m$.

% Figure~\ref{fig:meal_ndcg} indicates that across all models, we are able to predict the best for breakfast (B), which has an nDCG@5 scores much larger than that of the next-day set-up (Day). This is probably because breakfasts involve more users in repeat consumption to bring up higher prediction performance. For the other meals, the next-meal prediction is not as good as that of next day, with snack(S), lunch(L), and dinner(D) having descending order of predicted nDCG@5 among users. Especially, the mean nDCG@5 across users lunch and dinner are 0.0233 and 0.0211 respectively for the Global baseline, far poorer than the other models. This indicates that for users have little overlap in their food choices in these two "main meals".

% As shown above, model performances are consistently better for groups with higher repeat consumption under all contexts. The models are biased toward the groups with higher repeat consumption. This difference has an implication for health intervention, that we should make sure we can equally for all demographic subgroups, especially the groups tend to eat less healthy\cite{Achananuparp2018}.
% Males are more careless about healthy eating than females. In this MFP population, the algorithms are able to serve them coincidentally better in terms of food recommendation.
% In terms of age, younger adults need more attention than older adults. However, the algorithms can not serve them very well.
% In terms of locations, we are less able to predict accurately for regions which tend to eat unhealthy (Midwest and South). 
% For meal occasions, we surmise that people eat more unhealthy during lunch and dinner. More health intervention should be carried out during dinners, in which people socialize and care less about healthy eating. However, the algorithms are unable to achieve this.
% Overall, the algorithms more suitable for healthy eating intervention for the male groups. Under other context, the algorithms do not do well.

==> [DPH 2019] Repeat Food Consumption/data.tex <==
Popular food diary and health tracking applications, such as MyFitnessPal (MFP), Fitbit, etc., provide a useful and publicly available source of granular data suitable for the study of food consumption behaviors of individuals. In this study, we used a MyFitnessPal food diary dataset\footnote{\url{http://bit.ly/2XMywQO}} created by Weber and Achananuparp \cite{Weber2016}. The original dataset contains: (a) 
% 6,502,747 
6.5M
food diary entries collected from 
% 9,896 users 
9.9K users 
covering a 6-month period from September 2014 to April 2015; and (b) user profile information (e.g., gender, age, location, etc.) of 
% 8,794 users. 
8.8K users. 
Each food diary entry (a data row) consists of textual description of a food item and its portion size, meal occasion (e.g., breakfast, lunch, etc.), nutrition (e.g., calories, protein, fat, etc.), and a set of high-level food categories (e.g., meats, vegetables, etc.) and sub-categories (e.g., beef, wheat, etc.) annotated by the dataset creators. 
% This way of uniquely identify items is not accurate. To be done/explored in the follow-up:
% To reduce sparsity in the user-item consumption data caused by linguistic variation in the textual description of food diary entries, we identified unique food items by their food categories. That is, food diary entries sharing the exact same sets of categorical terms were considered containing the same food items. 
To reduce sparsity in the user-item consumption data, we removed keywords mentioning: (a) specific commercial entities, such as brand and restaurant names, and (b) quantities, from the textual description of food diary entries.
We further selected a subset of the original data from October 12, 2014 to March 14, 2015 (22 weeks) for their frequent activity level to be used in this study.

% After obtaining the food diary data, 
We performed the following data cleaning steps. First, we removed outlier entries such as those with negative portion sizes, food with calories higher than 3,000 kcal, and non-food entries such as ``quick add calories'' 
% (33,896, 0.52\% of all records).
(33.9K, 0.52\% of all records). Next, we removed entries containing auxiliary items, such as dietary supplements and condiments 
% (1,138,102, 17.50\%).
(1.1M, 17.50\%).
For the prediction task, we only considered records from meals with breakfast, lunch, dinner, or snack labels. Meals with other labels 
% (1,441,978, 22.17\%) 
(1.4M, 22.17\%)
were excluded. Lastly, we performed a p-core filtering by recursively removing: (a) food items that were not consumed by more than 5 users; and (b) users who consumed less than 20 remaining food items 
% (1,671,961, 25.71\%). 
(1.7M, 25.71\%).
After the data cleaning and preprocessing steps, the dataset contains 2.7M food diary entries involving 55K unique food items and 7.7K unique users as shown in Table~\ref{tbl:data_stats}. Demographically, a vast majority of users were female (82.62\%), young adults 18-44 years of age (79.09\%), and lived in the United States (71.72\%).

\begin{table}[thp]
\centering
\caption{Data statistics}
\label{tbl:data_stats}
\scalebox{0.9}{
\begin{tabular}{lr}
\toprule
% \midrule
\# users & 7,721 \\
\# items & 55,584 \\
\# meals & 1,149,692 \\
\# diary entries & 2,737,885 \\
% density & 0.64 \\
\# items per user (mean $\pm$ S.D.) & 115 $\pm$ 85.57 \\
\# items per user per day (mean $\pm$ S.D.) & 5.86 $\pm$ 3.57 \\
\% female & 82.62\% \\
\% 18-44 years old & 79.09\% \\
\% United States & 71.72\% \\
\bottomrule
\end{tabular}
}
\end{table}

% \subsection{Data Characteristics}
% \label{sec:data_char}
% Let us further examine the characteristics of our data. 
Figure~\ref{fig:user_trends} shows the number of active users -- those who recorded their food diary on any given day, over time (mean daily active users = 3,034). The data exhibit a clear cyclic pattern where the users tended to be more active on weekdays than weekends. Furthermore, fewer users continued to record food diaries during the holidays. For example, the numbers of daily active users decreased by 23.3\% and 24.3\% on Thanksgiving day and Christmas day, respectively. At the start of 2015, a large number of active users emerged, possibly due to the effect of the new year's resolution. 
% In particular, on the first Monday of 2015, the number of daily active users increased by 42\%. 
% The surge could be partly due to a common new year's resolution to lose weight.
% (from 2886 to 4098), Amongst these, 142 were new users. This is the largest expansion of user base.
% These were either newly registered users or existing users who became active again.
% other decreases: Muharram (14.3\%), Halloween (14.6\%), Christmas Eve (19.7\%)
% consider to introduce the concept of user base (users that ever active in the crawling period) and the concept of new users (users newly joined to the user base, who are either i) new to the MFP app or inactive during the earlier days of our crawling range)
% possible to include a plot for new user trends on the same graph (use y-axis on the right) 
Next, the food consumption pattern follows a near power-law distribution. Figure~\ref{fig:consumption_frequency} shows an empirical cumulative distribution function (CDF) plot of the food items recorded across all food diary entries (i.e., food consumptions). As we can see, up to 30\% of food items accounted for 80\% of food diary entries, suggesting that a small fraction of items tended to be reconsumed most of the time.

% 6*3 inches, bbox_inches='tight', pad_inches=0.0 => size: (517, 1124)
\begin{figure}[tp]
 \includegraphics[scale=0.45,center]{figures/ts_user_cnt.png}
 \caption{Number of active users over time}
 \label{fig:user_trends}
\end{figure}
% 6*3 inches, bbox_inches='tight', pad_inches=0.05 => size: (545, 1151)
\begin{figure}[tp]
 \includegraphics[scale=0.45,center]{figures/line_food.png}
 \caption{CDF of food items}
 \label{fig:consumption_frequency}
\end{figure}

% Item composition and variations section was moved to the backup folder /backup/item_composition.tex to make room for the modifications.
% \subsection{Item Composition and Variations}


==> [DPH 2019] Repeat Food Consumption/experiments.tex <==
% The ability to predict future food consumptions can be helpful in improving users' gastronomic experience through the recommendations of new food items which are relevant to the users' tastes and dietary preferences. More importantly, food recommender systems can also play a crucial role in facilitating healthy lifestyle change \cite{Trattner2017,Freyne2010}, serving as a behavior prediction component in online healthy eating intervention programs. 

% Historically, research in food recommender systems mainly focused on generating the recommended lists of novel food items (e.g., cooking recipes) from the users' past ratings of items independent of the consumption time and context. However, according to the findings shown in the previous section, 
Due to the novel and repeat consumption dynamics and the context-sensitive nature of food consumption, we argue that predicting a complete set of repeat and novel food items for the next consumption sessions is a more pertinent task for food recommender systems than the general rating prediction task, especially in the just-in-time health intervention scenario. Once the users' daily eating habits are learned, different behavioral interventions can be taken, for example, recommending healthier and similar substitutes to replace the less healthy but highly reconsumed items, recommending healthy novel items complementary to the basket of highly reconsumed items, etc. In addition, many state-of-the-art algorithms in food recommender systems, such as matrix factorization, are effective in recommending new items to the users, their performance in predicting both the repeat and novel food items for future consumptions is currently not known. Lastly, traditional food recommender systems often rely on the user-item rating data which may be scarce or difficult to obtain given the burden of data collection. 

Therefore, we present an offline experiment of \textit{just-in-time} food recommendation to investigate the effectiveness of many recommender system algorithms using \textit{implicit feedback} data in which only the historical consumptions and no rating data are provided. Specifically, we define the food recommendation task as generating the top-$N$ recommendation list for the \textit{next-day} consumption. Moreover, as food consumption behavior is highly context-sensitive, we further conduct a context-aware evaluation to examine the performance of different algorithms across subgroups of users based on their demographic attributes and contexts. The results of the context-aware evaluation will be discussed later in section \ref{sec:context}.


% Helena's old writing
% In this section, we asked the question -- given the consumption history of the user, what does the user eat next time? The understanding of what the user consume as time changes would be the foundation of the new food recommendation that further provide insights to intervene the eating behavior, thus help the user switch to a healthier diet. We tackled this question from two different perspectives. First, we examined what kind of recommender system would better catch the eating behavior. As we observed that the users on MyFitnessPal have a high tendency towards repeat consumption, would the models which emphasize capturing toward repeat consumption beat the others which are not?
% Second, we questioned if there is any weekly routine or weekend-specific effects on the user consumption. 

\subsection{Algorithms}
\label{sec:algo}
We compare the performance of eight algorithms in the just-in-time food recommendation evaluation. These algorithms can be categorized into 4 following groups: multinomial mixture models, sequential recommender models, latent-factor models, and rule-based methods.

\textbf{Multinomial Mixture Models}: Motivated by the recent success of the multinomial mixture model (\textbf{Mixture}) \cite{Kotzias2018}, which has been shown to outperform most state-of-the-art algorithms in several implicit-feedback recommendation tasks, we propose a time-weighted mixture model (\textbf{MixtureTW}) as a simple extension of \textbf{Mixture}. The original \textbf{Mixture} consists of two multinomial components that capture the balance between the \textit{individual} exploitation component ($\theta^I$) and the \textit{population} exploration component ($\theta^P$), i.e., the repeat and the novel consumptions, respectively. This exploration-exploitation framework seems naturally suitable for modeling the food consumption behaviors of individuals due to the inherently recurring nature of the data. In \textbf{Mixture}, the probability $P_{ij}$ of user $u_i$ consuming item $f_j$ is formally defined as:

\begin{equation}
\label{eq:mixture}
    P_{ij} = \pi_i \theta^I_{ij} + (1 - \pi_i ) \theta^P_j
\end{equation}

where the personalized mixture weight $\pi_i$ represents the trade-off between the two components $\theta^I_{ij} = \frac{C_{ij}}{C_i}$ and $\theta^P_j = \frac{C_j + 1}{C + |F|}$; $C_{ij}$ denotes the user-item consumption count of user $u_i$ and item $f_j$; $F$ denotes the set of all food items. The Expectation-Maximization (EM) algorithm is used to learn $\pi_i$ from the training and validation data \cite{Kotzias2018}.

In \textbf{MixtureTW}, we incorporate the idea of time-weighted recommender systems \cite{Ding2005} into \textbf{Mixture} by decaying user-item consumption counts over time such that recent consumption counts are weighted higher than old consumption counts. Specifically, let $T$ be the most recent time step, the user-item consumption count $C_{ij}$ for the time steps $[1, T]$ is discounted by a decay rate $\lambda \in (0, 1)$ as follow: 

\begin{equation}
\label{eq:decay}
C_{ij} = \sum_{t=1}^{T} \lambda^{T - t} c_{ij}^t
\end{equation}.

% \begin{equation}
% \label{eq:decay}
% C^{[t_l,t_r)}_{ij} = \sum_{t \in [t_l, t_r)} \lambda^{t_r + 1 - t} c^t_{ij}    
% \end{equation}

% \begin{equation}
% C_{ij} = \sum_{t=1}^{\vert T \vert} \lambda^{\vert T \vert-t} C_{ij}(t)
% \end{equation}

% Thus, for the training period of $[t_k,t_r)$, $\theta^I_{ij} = \frac{C_{ij}}{C_j} $,
% $\theta^P_{j} = \frac{C_j + 1}{C + |F|}$.

% Next, we adopted the recently proposed \cite{Kotzias2018} mixture model (\textbf{Mixture}), which explicitly considers the balance between novel (exploration) and repeat (exploitation) consumption behaviors, as one of the competitive baselines. The mixture model computes the probability $P_{ij}$ of user $u_i$ consuming item $f_j$ by learning the personalized mixture weight $\pi_i$ that controls the trade-off between repeat (exploitation) and novel (exploration) consumption components in the validation data. It has been shown to outperform many state-of-the-art algorithms, including NMF, in a variety of tasks, such as music recommendation, geolocation check-ins prediction, etc. \cite{Kotzias2018}. In the experiments, we used the original implementation of the mixture model\footnote{https://github.com/UCIDataLab/repeat-consumption}. 

where $c_{ij}^t$ is the number of times user $u_i$ consumed item $f_j$ in the time step $t$. Similar time weighting is applied to other consumption count data, e.g., $C_i$, $C_j$, etc., to derive $\theta^I_{ij}$ and $\theta^P_j$.

In the experiment, we consider both \textbf{MixtureTW} and \textbf{Mixture} as competitive algorithms. Our implementations of \textbf{MixtureTW} and \textbf{Mixture} are based on the original authors' code\footnote{https://github.com/UCIDataLab/repeat-consumption}.

\textbf{Sequential Recommender Models}: Additionally, we employ a well-known Factorizing Personalized Markov Chains algorithm (\textbf{FPMC}) \cite{Rendle2010} as a representative baseline for sequential recommender systems. \textbf{FPMC} takes into account both sequential information of items in different time steps and general user preferences when generating recommendations. In the experiment, we modified a python implementation of \textbf{FPMC}\footnote{https://github.com/khesui/FPMC} (v.0.1) to allow for variable-sized baskets.

\textbf{Latent-Factor Models}: Next, we include three latent factor models widely-used in the implicit-feedback recommender systems, i.e., non-negative matrix factorization (\textbf{NMF}), hierarchical Poisson factorization (\textbf{HPF}) \cite{Gopalan2015}, and latent Dirichlet allocation (\textbf{LDA}) \cite{Blei2003}. These algorithms have been empirically shown to perform effectively in both the user-item rating prediction and the implicit-feedback general recommendation tasks \cite{Gopalan2015,Kotzias2018,Trattner2017}. In the experiment, we used the scikit-learn\footnote{https://scikit-learn.org} (v.0.20) implementations of \textbf{NMF} and \textbf{LDA} and the hpfrec\footnote{https://github.com/david-cortes/hpfrec} (v.0.2.2) implementation of \textbf{HPF}.

\textbf{Rule-Based Methods}: Lastly, we define two rule-based algorithms as simple baselines: global popularity (\textbf{Global}) and personal favourite (\textbf{Personal}). \textbf{Global} is a naive baseline in which each item $f_j$ is assigned a score proportional to its global consumption frequency $n_j$ in the training set. Thus, every user was recommended the same set of globally popular items in each session. Next, \textbf{Personal} is another naive baseline where a score of user $u_i$ consuming item $f_j$ is proportional to the consumption frequency $n_{ij}$ from $u_i$'s past consumptions of $f_j$ in the training set. That is, the method simply assumes that the users always reconsumed their personally favourite items and never tried new items, i.e., exploitation-only behavior.

% Longer description
% We compare the performance of six algorithms in the just-in-time food recommendation evaluation. Firstly, we adopted the recently proposed \cite{Kotzias2018} mixture model (Mixture), which explicitly considers the balance between novel (exploration) and repeat (exploitation) consumption behaviors, as one of the competitive baselines. Next, we included latent factor models commonly used in recommender systems with implicit feedback data, such as non-negative matrix factorization (NMF), hierarchical Poisson factorization (HPF) \cite{Gopalan2015}, and latent Dirichlet allocation (LDA) \cite{Blei2003}. Lastly, we defined two simple rule-based algorithms as naive baselines: global popularity (Global) and personal favourite (Personal).

% \textbf{Mixture}: The mixture model computes the probability $P_ij$ of user $u_i$ consuming item $f_j$ by learning the personalized mixture weight $\pi_i$ that controls the trade-off between repeat (exploitation) and novel (exploration) consumption components in the training data. It is computationally efficient and has been shown to outperform many state-of-the-art algorithms, including NMF, in both a variety of online and offline tasks, such as music recommendation, geolocation check-ins prediction, etc. \cite{Kotzias2018}. In the experiments, we used the original Python implementation of the mixture model\footnote{https://github.com/UCIDataLab/repeat-consumption}.

% \textbf{NMF}: NMF is one of the most widely-used algorithms in recommender systems. Recently, it has been suggested that NMF does not perform well when the consumption data contain both repeat and novel items due to its tendency to oversmooth \cite{Kotzias2018}. In the experiments, we used a Python implementation of NMF in the scikit-learn library\footnote{https://scikit-learn.org}.
% % In NMF, the user-item preferences are modeled as non-negative vectors in a low-dimensional space. These latent vectors are randomly initialized and modified via an alternating multiplicative update rule to minimize the Frobenius norm between the actual and the modeled consumption frequency matrices.  

% \textbf{HPF}: Unlike NMF, HPF assumes that the user-item consumption matrix is drawn from the Poisson distribution and places Gamma priors on both the latent user and latent item factors. It was empirically shown to outperform state-of-the-art algorithms on many recommendation tasks with long-tailed consumption data \cite{Gopalan2015}. In the experiments, we used the python implementation\footnote{https://github.com/david-cortes/hpfrec} of HPF.

% \textbf{LDA}: LDA is a well-known graphical model for topic modelling. Interestingly, it was shown to perform effectively as a general-purpose matrix factorization method in several recommendation tasks \cite{Gopalan2015,Trattner2017,Kotzias2018}. In this study, we used a Python implementation of LDA in the scikit-learn library.
% % we used a Python implementation of LDA in the gensim library\footnote{https://radimrehurek.com/gensim/}.

% \textbf{Global}: Global is a naive baseline in which each item $f_j$ is assigned a score proportional to its global consumption frequency $n_j$ in the training set. Thus, every user was recommended the same set of globally popular items in each session.

% \textbf{Personal}: Personal is another naive baseline where a score of user $u_i$ consuming item $f_j$ is proportional to the consumption frequency $n_{ij}$ from $u_i$'s past consumptions of $f_j$ in the training set. That is, the model simply assumes that the users always reconsumed their personally favourite items and never tried new items, i.e., exploitation-only behavior.

\subsection{Experimental Protocols}
\label{sec:exp_protocols}
We used the MFP dataset previously described in Table~\ref{tbl:data_stats} in the experiment. The dataset was split into 146 sliding-window sessions. Each experiment session contains 9 days (or 9 time steps) of food consumption sequence data and the next session was incremented by one time step from the previous session. In each session, data at the most recent time step $t$ were used as a held-out test set for evaluation, those at $t-1$ were used as a validation set for optimizing hyperparameters, and those at $[t-8, t-1)$ were used as a training set.
% , to preserve only the most recent food items consumed. 
Given a set of all food items in the training set $F$, for each session, the goal is to estimate for each user $u_i$, $\theta_i$ = [$\theta_{i1}$, \dots, $\theta_{i|F|}$], $\sum_{f_j \in F} \theta_{ij}$ = 1 where $\theta_{ij}$ is the probability that user $u_i$ consumed item $f_j$ at time step $t$.
% , conditioned on the event that $u_i$ consumed some items at time step $t$. 
% data is further filtered, and why
% The item set $F$ for a session was restricted to those existing in the training data. 
Moreover, we removed from the test set (i) unseen items (those not existing in the training set) and (ii) unseen users (those not existing in the training and the validation sets) to ensure that the mixture models were able to estimate a personalized mixture weight $\pi_i$ for all the users in the test set. On average, 3.6K unseen items (S.D. = 928) and 595 unseen users (S.D. = 252) were removed per session.
The statistics of the dataset used in the experiment are summarized in Table \ref{tbl:stats2}.
% The user set $U$ in a session was defined by all the training, validation, and testing data in the session. The training and testing sets are indicative of the users we have to train and to predict. The validation is also required to tune user mixture weight $\pi_i$ for the mixture model.
% Therefore, we removed items in the test set which were unseen in the training set (3601 $\pm$ 928), and users which were unseen in the training and the validation sets (595 $\pm$ 252) per session. 

For the training data used in all algorithms (except \textbf{HPF}), the user-item consumption frequency matrix is L1 normalized, such that the item consumption frequencies add up to 1 for each user. This allows the algorithms to be more robust to outliers. Since \textbf{HPF} inherently models the skew in item popularity, we used the original user-item consumption frequency matrix as input for \textbf{HPF}.
% and  normalized the mean posterior expected Poisson parameters, $score_{ui}$ of item $f_j$ for each user $u_i$ to get the predicted consumption probability $\theta_{ij}$. 
% For HPF,  default stop_crit='train-llk', we used stop_crit='val-llk',.
% Default maxiter=100, we used maxiter=500,
% Default reindex=True, ours reindex=False. (This does not affect the results.) 
Next, we used the default hyperparameters in the respective packages for \textbf{NMF}, \textbf{HPF}, \textbf{LDA}, and \textbf{FPMC} and evaluated different numbers of latent factors using a subset of the experiment data spanning 3 days (January 20 - 22 of 2015). Lastly, we optimally set the number of latent factors for 
\textbf{NMF}, \textbf{HPF}, \textbf{LDA}, and \textbf{FPMC} to 100, 500, 50, and 500, % same param as randomly selecting 5 sessions, see below
respectively, for all sessions. For \textbf{MixtureTW}, the decay weight $\lambda$ was optimally tuned for each test session.
% For each test session, tune with range (0.0, 1.0, 0.05), report average lambda.

% LDA performence is the same  when training the model with the normalized count matrix and when using raw counts

% In the tuning, we randomly selected 5 sessions (test dates fall on 2014-10-20. 2014-11-06, 2014-11-22, 2015-01-20, 2015-02-08). For all sessions, if we evaluate on the valuation set with nDCG@5, 50 factors perform the best for LDA among 2, 10, 20, 50, 100, 200, 500, 700, and 1000.
% NMF and HPF have their performance increased with decreasing rate as the number of factor increases, but the time required to construct the model grows exponentially.

% We heuristically set the training size as seven days, validation size as one day and testing size as one day. In other words, we let the T = 7 and $\Delta {t}$ = 1. In the testing set, we remove the item which is unseen in the training set and the user which is unseen in the training and validation set, as in Table~\ref{tbl:expeiment_data_stats}. For the matrix factorization-based models, we decide the factor numbers by experimenting with a small set of epochs (test dates being 20 to 22 Jan 2015). NMF performs The factor number when the number of factor increases, and the time required to construct the model grows much faster than the performance increase. For LDA, factor number of 50 gives the best results for all sample epochs, any larger or smaller give worse results. Finally, we set the factor number as 50 for LDA model, 100 for NMF model, and 500 in the HPF model for all epochs.
% We aim to predict the probability of food items to be consumed by all users in a period, given the historical consumption frequency of the food items by the users. We assume a scenario where the data are collected and aggregated over some time period T (e.g., one week of data), and our goal is to generalize from the historical data and make predictions for some time period ($T$, $T$ + $\Delta {t}$), where $\Delta {t}$ is some window of, e.g., corresponding to the next day or next meal. The data input is an aggregated consumption matrix. It is an array of (N x 3), where each row is the (row, column, value) triplet correspond to (user, item, consumption frequency), and N is the number of entries in the array.

\begin{table}[thp]
\centering
\caption{Experiment data statistics}
\label{tbl:stats2}
\scalebox{0.9}{
\begin{tabular}{lr}
\toprule
% Users & items stats were already known. Not true: some users and items are never present for the prediction task.
% \# users & 7,608 \\
% \# items & 55,584 \\
\# sessions & 146 \\
\# users/session (mean $\pm$ S.D.) & 2,461 $\pm$ 683 \\
\# items/session (mean $\pm$ S.D.) & 23,651 $\pm$ 4,385 \\
% Previously very small s.d.: averaged over users per session, then averaged over the sessions. Currently changed to average across all users and sessions directly. 
\# items/user in training (mean $\pm$ S.D.) & 21.81 $\pm$ 10.64 \\
% (21.81082, 10.641)
\# items/user in validation (mean $\pm$ S.D.) &  5.27 $\pm$ 3.16 \\
% (5.27627, 3.15702)
\# items/user in testing (mean $\pm$ S.D.) & 5.13 $\pm$ 3.12 \\
% (5.12529, 3.11829)
\# novel items/user in testing (mean $\pm$ S.D.) & 3.55 $\pm$ 2.51 \\
% (3.54512, 2.50984)
\# repeat items/user in testing (mean $\pm$ S.D.) & 1.58 $\pm$ 1.89 \\
% (1.58018, 1.89655)
\bottomrule
\end{tabular}
}
\end{table}

In addition, to obtain the meal-specific food recommendation results for the context-aware evaluation, we first split the experiment data into 4 disjoint subsets for breakfast, lunch, dinner, and snack. Then, the same protocols described earlier were performed on each meal-specific subset.
% , i.e., the training, validation, and test sets were limited to the consumption data of the same meal occasion for each session. 
Due to space constraints, we only reported their results in section \ref{sec:context}. 

\subsection{Evaluation Metrics}
We used three standard metrics commonly used in the implicit-feedback recommendation evaluation: recall, precision, and normalized discounted cumulative gain (nDCG), to measure the effectiveness of different algorithms in generating the top-$N$ recommendation lists. Firstly, \textbf{recall@N} is defined as the proportion of actual consumption in the test set was identified correctly in the top-$N$ recommendation list, over all items actually consumed by $u_i$, i.e., the size of the test set. Particularly, we adopted the definition of weighted recall used in Kotzias et al. \cite{Kotzias2018} shown in equation~\ref{eq:recall@N}.

\begin{equation}
\label{eq:recall@N}
% \resizebox{0.75\hsize}{!}{$
\mathrm{Recall@N} = \frac{1}{|U|} \sum_{i \in U} \sum_{j}\frac{n_{i,j}\cdot\mathbf{I}\big(rank(i,j)\leq{N}\big)}{\sum_{j}n_{i,j}}
% $}
\end{equation}

Next, \textbf{precision@N} is defined as the fraction of correctly recommended items in the top-$N$ recommendation list. As the size of test set varies for different users, precision@N may be underestimated for some users who generally consumed fewer $n$ items. Lastly, \textbf{nDCG@N} is defined as a discounted cumulative gain (DCG) of items in the top-$N$ recommendation list normalized by the ideal discounted cumulative gain (IDCG), which is obtained by computing DCG for items in the test set sorted descendingly by their consumption frequency $n_{ij}$ in the test set. As nDCG considers multiple levels of relevance, it is more sensitive to the relevance of higher ranked items.

For each algorithm, we first computed scores for each user $u_i$ in each session and averaged the results across all users. Then, we averaged the scores across all sessions to obtain the average performance for each algorithm. The values for all metrics range from 0 (worst) to 1 (best). In the experiment, we set $N = 5$ for the \textit{all-item} evaluation setup and $N = 3$ for the \textit{novel item-only} evaluation setup. Lastly, to evaluate the statistical differences between the performance of different algorithms (RQ2) and the context-specific performance across different groups (RQ3), we performed Kruskal-Wallis H test with Dunn's multiple comparison test at the significance levels of 0.01 and 0.05.

% Longer version
% We used three standard evaluation metrics: recall, precision, and normalized discounted cumulative gain (nDCG), to measure the effectiveness of different algorithms in generating the top-$N$ recommendation lists. For each algorithm, we first computed scores for each user $u_i$ in each session and averaged the results across all users. Lastly, we averaged the scores across all sessions to obtain the average performance for each algorithm. The values for all metrics range from 0 (worst) to 1 (best). In the experiments, we set $n = 5$.

% % evaluate the actual consumption frequency $n_{ij}$ in test data against the predicted consumption probability $\theta_{ij}$

% \textbf{Recall@N} is defined as proportion of actual consumption in the test set was identified correctly in the top-$N$ recommendation list, over all items actually consumed by $u_i$, i.e., the size of the test set.

% \begin{equation}
% \label{eq:recall@N}
% % \resizebox{0.75\hsize}{!}{$
% \mathrm{Recall@N} = \frac{1}{|U|} \sum_{i \in U} \sum_{j}\frac{n_{i,j}\cdot\mathbf{I}\big(rank(i,j)\leq{N}\big)}{\sum_{j}n_{i,j}}
% % $}
% \end{equation}

% \textbf{Precision@N} is defined as the fraction of correctly recommended items in the top-$N$ recommendation list. As the size of test set varies for different users, precision@N may be underestimated for some users who generally consumed fewer $n$ items.

% \begin{equation}
% \label{eq:prec@N}
% % \resizebox{0.75\hsize}{!}{$
% \mathrm{Precision@N}=\frac{1}{|U|}\sum_{i \in U}
% \sum_{j} \frac{\mathbf{I}\big(rank(i,j)\leq{N}\big)}{N}
% % $}
% \end{equation}

% \textbf{nDCG@N} is defined as a discounted cumulative gain (DCG) of items in the top-$N$ recommendation list normalized by ideal discounted cumulative gain (IDCG), which is obtained by computing DCG for items in the test set sorted descendingly by their consumption frequency $n_{ij}$ in the test set. As nDCG considers multiple level of relevance, it is more sensitive to the relevance of higher ranked items. 
% % This characteristic makes it highly desirable for measuring ranking quality in recommender systems as most users rarely look past the ﬁrst few items on a recommendation list so the relevance of items at the top positions are far more important than those at low positions.

% \begin{equation}
% \label{eq:dcg@N_i}
% % \resizebox{0.75\hsize}{!}{$
% \mathrm{DCG@N(i)} = \sum_{j} \frac{(2^{n_{i,j}} - 1)\cdot\mathbf{I}\big(rank(i,j)\leq{N}\big)}{\log_2^{(rank(i,j)+1)}}
% % $}
% \end{equation}

% \begin{equation}
% \label{eq:ndcg@N_i}
% % \resizebox{0.5\hsize}{!}{$
% \mathrm{nDCG@N(i)} = \frac{DCG@N(i)}{IDCG@N(i)}
% % $}
% \end{equation}

% \begin{equation}
% \label{eq:ndcg@N}
% % \resizebox{0.5\hsize}{!}{$
% \mathrm{nDCG@N} = \frac{1}{|U|} \sum_{i \in U} nDCG@N(i)
% % $}
% \end{equation}
\subsection{Results \& Discussion}
\label{sec:results}
Table~\ref{tbl:recc_results} displays the average recall@5, precision@5, and nDCG@5 across all 146 experiment sessions for the eight algorithms. Overall, there is a significant difference in the performance of different algorithms (p \textless 0.01). 
Particularly, \textbf{MixtureTW} significantly outperformed the other algorithms in all metrics (p \textless 0.01), e.g., +74.2\% of \textbf{NMF} in nDCG@5. 
% Moreover, \textbf{Mixture} was the second best algorithm. 
The average mixture weights $\pi_i$ of \textbf{MixtureTW} and \textbf{Mixture} across all sessions was 
% 0.669 (S.D. = 0.045)
0.667 (S.D. = 0.168), indicating that the individual exploitation component ($\theta^I$) was generally more important than the population exploration component ($\theta^P$). In addition, the mean decay factor $\lambda$ for \textbf{MixtureTW} was 0.812 (S.D. = 0.046), suggesting a strong recency bias. 
% towards the recent consumptions
% of habitual consumption, as recently consumed food items play a larger role in determining the near-future consumptions than older food items. 
The superior performance of the multinomial mixture models over the latent-factor models in our experiment is consistent with the results from the prior research \cite{Kotzias2018}.
% the previous online consumption experiment \cite{Kotzias2018}.

\begin{table}[thp]
\centering
\caption{Performance (mean $\pm$ standard deviation) of different algorithms in generating complete recommendations (repeat + novel) across all sessions. The best results are in bold.}
\label{tbl:recc_results}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method & recall@5 & precision@5 & nDCG@5 \\
\midrule
\textbf{MixtureTW} &  \textbf{0.389} $\pm$ 0.029 &  \textbf{0.352} $\pm$ 0.039 &  \textbf{0.465} $\pm$ 0.038 \\
\textbf{Mixture} & 0.370 $\pm$ 0.026 & 0.337 $\pm$ 0.035 & 0.446 $\pm$ 0.034 \\
\midrule
\textbf{FPMC} & 0.355 $\pm$ 0.027 & 0.321 $\pm$ 0.034 & 0.414 $\pm$ 0.034 \\
\midrule
\textbf{NMF}      &  0.185 $\pm$ 0.009 &  0.176 $\pm$ 0.014 &  0.267 $\pm$ 0.012 \\
\textbf{HPF} & 0.099 $\pm$ 0.005 & 0.102 $\pm$ 0.010 & 0.143 $\pm$ 0.002 \\
\textbf{LDA}      &  0.071 $\pm$ 0.013 &  0.060 $\pm$ 0.005 &  0.083 $\pm$ 0.009 \\
\midrule
\textbf{Global}   &  0.054 $\pm$ 0.004 &  0.052 $\pm$ 0.004 &  0.073 $\pm$ 0.004 \\
\textbf{Personal} &  0.366 $\pm$ 0.026 &  0.333 $\pm$ 0.035 &  0.440 $\pm$ 0.034 \\
\bottomrule
\end{tabular}
}
\end{table}

Surprisingly, the popular sequential recommender model, \textbf{FPMC}, was not as effective as \textbf{MixtureTW} and \textbf{Mixture}. This might be due to the highly repetitive nature of food consumption in the MFP dataset. For \textbf{FPMC}, the item sequence information from the first-order Markov chains, which is treated as equally important as user preferences, may not be very helpful for the highly repetitive dataset.
% biased towards novel items, works well empirically for FPMC
% I found a paper Modeling Item-Specific Temporal Dynamics of Repeat Consumption for Recommender Systems(by a Tsinghua Min ZHANG's group, WWW'19), which considers FPMC able to "make holistic item recommendation", which differs from algorithms, such as BPR-MF, which "do not take repeat consumption into consideration".
% In the experiment results, compares BPR-MF and FPMC. FPMC has higher nDCG than BPR-MF for datasets with less repeat consumption (14-21\%), whereas FPMC is worse than BPR for a datasets with very heavy repeat consumption (90\%).
Amongst the latent-factor models, \textbf{NMF} performed better than \textbf{HPF} and \textbf{LDA}. The relative performance of the latent-factor models in our experiment differs from those reported in the previous studies \cite{Gopalan2015,Kotzias2018}.
% , where \textbf{HPF} and \textbf{LDA} tended to be more effective than \textbf{NMF} in the implicit-feedback recommendation task. 
This inconsistency could possibly occur due to: (1) the differences in the experiment setup;
% , i.e., just-in-time recommendation vs. general recommendation
 and (2) the differences in data characteristics and user behavior.
% , i.e., offline food consumptions vs. online media consumptions. Unsurprisingly, \textbf{Global} is the least effective algorithm. 
Lastly, the simple \textbf{Personal} baseline performed fairly competitively (-5.4\% of \textbf{MixtureTW} in nDCG@5). Again, this might be explained by the heavily repetitive nature of the food consumption data.

% the performance of \textbf{Personal} is virtually identical to \textbf{Mixture} (-1.3\% of \textbf{Mixture} in nDCG@5). The highly repetitive nature of food consumption may explain why \textbf{Personal} was as effective as \textbf{Mixture}.
% Moreover, the near-identical results also show that \textbf{Mixture} was still relatively less effective in predicting novel items than predicting repeat items.
% add $\pi_i$ for MixtureTW:            mean = 0.669298876121923, s.d. = 0.04506604405985309, 
% which is about the same for Mixture:  mean = 0.6693948464505173, s.d. = 0.04499661722572324


% Although the prediction accuracy are much higher compared to similar recommendation tasks such as movie or music recommendation, the recommendations are not ready for adoption for users. 
% cite if necessary, for low performance
% @inproceedings{Vargas2013,
%   title={Exploiting the diversity of user preferences for recommendation},
%   author={Vargas, Sa{\'u}l and Castells, Pablo},
%   booktitle={Proceedings of the 10th conference on open research areas in information retrieval},
%   pages={129--136},
%   year={2013},
%   organization={LE CENTRE DE HAUTES ETUDES INTERNATIONALES D'INFORMATIQUE DOCUMENTAIRE}
% }

While \textbf{MixtureTW} was the most effective in predicting next-day food consumptions, compared to the other methods, it performed rather poorly in predicting novel consumptions. Specifically, we examined the recommended lists of food items used in the main evaluation (Table \ref{tbl:recc_results}) and measured the average recall@3, precision@3, and nDCG@3 of the subsets of \textit{novel item-only} recommendations. As shown in Table \ref{tbl:novel_results_3}, most algorithms failed to correctly identify a few novel food items from a large set of approximately 23K items in the training set -- a much more challenging setup than the typical novel recommendation task, most of the time. 
% In this case, \textbf{NMF} significantly outperformed all the other algorithms (p \textless 0.01).
% Running: evaluate performance for top 100 predictions

% !! new table: performance of all models: novel items only -> we may be able to take care of the repeat consumption, another model may be better in predicting novel food consumption
% Table~\ref{tbl:novel_results_3} displays the average recall@3, precision@3, and nDCG@3 across all 146 experiment sessions for the eight algorithms for recommending novel items only. 
% Overall, there is a significant difference in the performance of different algorithms (p \textless 0.01), and NMF outperforms the other algorithms. 
% Here, as Mixture only evaluates the novel items to each user, it would be the same as Global. 
% Personal is just slightly more than 0 as it ranks all novel item equally.
% MixtureTW is not statistically different from Mixture(Global) and LDA.

% some stats for whether the models are statistically different in terms of nDCG@3
% => MixtureTW is not different from Mixture, LDA and Global.
% => Mixture is not different from LDA and Global.
% => LDA is not different from HPF, Global
% 1.3108533387489937e-157
% mixture_decay_model [False  True  True  True False  True False]
% mixture_decay_model [1.   0.   0.   0.04 0.06 0.   1.  ]
% mixture_model [ True  True  True False  True False]
% mixture_model [0.    0.    0.039 0.058 0.    1.   ]
% fpmc_model [ True  True  True  True  True]
% fpmc_model [0.    0.003 0.002 0.    0.   ]
% nmf_model [ True  True  True  True]
% nmf_model [0. 0. 0. 0.]
% hpf_model [False  True  True]
% hpf_model [1.    0.    0.039]
% lda_model [ True False]
% lda_model [0.    0.058]
% personal_model [ True]
% personal_model [0.]


\begin{table}[thp]
\centering
\caption{Performance (mean $\pm$ standard deviation) of different algorithms in generating novel item-only recommendations across all sessions. The best results are in bold.}
\label{tbl:novel_results_3}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method &                      recall@3 &                   precision@3 &                        nDCG@3 \\
\midrule
\textbf{MixtureTW} &           0.00464 $\pm$ 0.001 &           0.00788 $\pm$ 0.002 &           0.00732 $\pm$ 0.001 \\
\textbf{Mixture}   &           0.00463 $\pm$ 0.001 &           0.00790 $\pm$ 0.002 &           0.00732 $\pm$ 0.001 \\
\midrule
\textbf{FPMC}      &           0.00286 $\pm$ 0.001 &           0.00576 $\pm$ 0.001 &           0.00560 $\pm$ 0.001 \\
\midrule
\textbf{NMF}       &  \textbf{0.03486} $\pm$ 0.005 &  \textbf{0.05970} $\pm$ 0.010 &  \textbf{0.07354} $\pm$ 0.012 \\
\textbf{HPF}       &           0.00409 $\pm$ 0.001 &           0.00702 $\pm$ 0.002 &           0.00657 $\pm$ 0.001 \\
\textbf{LDA}       &           0.00405 $\pm$ 0.001 &           0.00694 $\pm$ 0.002 &           0.00655 $\pm$ 0.001 \\
\midrule
\textbf{Global}    &           0.00463 $\pm$ 0.001 &           0.00790 $\pm$ 0.002 &           0.00732 $\pm$ 0.001 \\
\textbf{Personal}  &           0.00013 $\pm$ 0.000 &           0.00022 $\pm$ 0.000 &           0.00021 $\pm$ 0.000 \\
\bottomrule
\end{tabular}
}
\end{table}

% Summary paragraph
% [Aek's] Try to directly answer RQ2:
% - Which algorithm is the most effective? How did existing SOTA (FPMC, NMF, LDA) perform?
% - Other salient observations from the experiment? Maybe insights from the novel item-only evaluation.
\textbf{Summary of Findings}: The effectiveness of the eight recommender algorithms in the just-in-time implicit food recommendation greatly varied from 0.465 - 0.073 according to the nDCG@5 metrics. The multinomial mixture models (\textbf{MixtureTW} and \textbf{Mixture}), which explicitly considered the balance of the repeat and novel consumptions, were the most effective methods in predicting the individuals' next-day food consumptions. Moreover, \textbf{MixtureTW} significantly outperformed \textbf{Mixture} by incorporating the recency bias in decaying consumption count data over time. The state-of-the-art sequential recommender (\textbf{FPMC}) and the general recommender systems (\textbf{NMF}, \textbf{HPF}, and \textbf{LDA}) all performed poorly overall. Lastly, all algorithms were not effective in predicting next-day novel consumptions. The results are generally consistent with prior research \cite{Anderson2014,Kotzias2018} and emphasize the challenging nature of the just-in-time food recommendation task.

% results for top-100 predictions: recall@100 ranges from 0.00439 (Personal) to 0.08377 (NMF).
%\begin{tabular}{llll}
% \toprule
% Method &                    recall@100 &                 precision@100 &                      nDCG@100 \\
% \midrule
% MixtureTW &           0.04391 $\pm$ 0.006 &           0.00235 $\pm$ 0.000 &           0.01989 $\pm$ 0.003 \\
% Mixture   &           0.04380 $\pm$ 0.006 &           0.00235 $\pm$ 0.000 &           0.01984 $\pm$ 0.003 \\
% FPMC      &           0.03174 $\pm$ 0.004 &           0.00181 $\pm$ 0.000 &           0.01421 $\pm$ 0.002 \\
% NMF       &  \textbf{0.08377} $\pm$ 0.011 &  \textbf{0.00367} $\pm$ 0.000 &  \textbf{0.06658} $\pm$ 0.008 \\
% HPF       &           0.04175 $\pm$ 0.006 &           0.00224 $\pm$ 0.000 &           0.01886 $\pm$ 0.002 \\
% LDA       &           0.03339 $\pm$ 0.005 &           0.00184 $\pm$ 0.000 &           0.01600 $\pm$ 0.002 \\
% Global    &           0.04380 $\pm$ 0.006 &           0.00235 $\pm$ 0.000 &           0.01984 $\pm$ 0.003 \\
% Personal  &           0.00439 $\pm$ 0.001 &           0.00022 $\pm$ 0.000 &           0.00147 $\pm$ 0.000 \\
% \bottomrule
% \end{tabular}



% and confirm past findings regarding the strong recency bias of habitual consumptions \cite{Anderson2014} 
% and the oversmoothing tendency of matrix factorization algorithms to overestimate the probability of new items \cite{Kotzias2018}.
% \textbf{RQ2:} \textit{What is the effectiveness of different state-of-the-art implicit recommender systems in predict daily food consumption patterns of individuals in a just-in-time recommendation setting
% - Which algorithm is the most effective? How did existing SOTA (FPMC, NMF, LDA) perform?
% \textbf{MixtureTW} is the most effective algorithm in predicting next-day food consumption. The state-of-the-art implicit recommender systems which incorporate repeat consumption information and can make holistic item recommendation, such as Mixture and FPMC, generally outperforms the method which do not take repeat consumption into consideration, such as NMF, HPF and LDA). 
% - Other salient observations from the experiment? Maybe insights from the novel item-only evaluation.
% NMF is the most effective for predicting novel consumption, possibly due to the directly reflection the features of the user communities.
% @inproceedings{Zhang2006,
%   title={Learning from incomplete ratings using non-negative matrix factorization},
%   author={Zhang, Sheng and Wang, Weihong and Ford, James and Makedon, Fillia},
%   booktitle={Proceedings of the 2006 SIAM international conference on data mining},
%   pages={549--553},
%   year={2006},
%   organization={SIAM}
% }
% "One advantage of the NMF-based CF algorithms is
% that the coordinates obtained via NMF directly reflect
% the features of the user communities."

% [Evaluation on top 5 items predicted.]
% % Table~\ref{tbl:novel_results} displays the average recall@5, precision@5, and nDCG@5 across all 146 experiment sessions for the eight algorithms for recommending novel items only. Overall, there is a significant difference in the performance of different algorithms (p \textless 0.01), and NMF outperforms the other algorithms. Here, Mixture is the same as Global. Personal is just slightly more than 0 as we give equal probability for any novel item.

% results for top-5 predictions
% \begin{table}[thp]
% \centering
% \caption{Performance (mean $\pm$ standard deviation) of different algorithms in generating novel item-only recommendations across all sessions. The best results are in bold.}
% \label{tbl:novel_results}
% \scalebox{0.85}{
% \begin{tabular}{lccc}
% \toprule
% Method &                      recall@5 &                   precision@5 &                        nDCG@5 \\
% \midrule
% \textbf{MixtureTW}     &           0.00716 $\pm$ 0.001 &           0.00761 $\pm$ 0.001 &           0.00792 $\pm$ 0.001 \\
% \textbf{Mixture}       &           0.00713 $\pm$ 0.001 &           0.00758 $\pm$ 0.001 &           0.00790 $\pm$ 0.001 \\
% \midrule
% \textbf{FPMC}          &           0.00440 $\pm$ 0.001 &           0.00527 $\pm$ 0.001 &           0.00565 $\pm$ 0.001 \\
% \midrule
% \textbf{NMF}           &  \textbf{0.03826} $\pm$ 0.005 &  \textbf{0.03877} $\pm$ 0.006 &  \textbf{0.06100} $\pm$ 0.009 \\
% \textbf{HPF}           &           0.00657 $\pm$ 0.001 &           0.00706 $\pm$ 0.001 &           0.00728 $\pm$ 0.001 \\
% \textbf{LDA}           &           0.00626 $\pm$ 0.001 &           0.00671 $\pm$ 0.001 &           0.00705 $\pm$ 0.001 \\
% \midrule
% \textbf{Global}        &           0.00713 $\pm$ 0.001 &           0.00758 $\pm$ 0.001 &           0.00790 $\pm$ 0.001 \\
% \textbf{Personal}      &           0.00022 $\pm$ 0.000 &           0.00022 $\pm$ 0.000 &           0.00024 $\pm$ 0.000 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% [Tuning MixtureTW.]
%ndcg vs lambda for a few sessions, similar to https://docs.google.com/presentation/d/1oeK5faz79286j6aIAkHc61s4uFft4pMQpGlQRIqVFhQ/edit#slide=id.g563f952035_0_50
% script is running, for randonly selected 5 sessions {'28': '2014-10-20',
%  '45': '2014-11-06',
%  '61': '2014-11-22',
%  '120': '2015-01-20',
%  '139': '2015-02-08'} - done

==> [DPH 2019] Repeat Food Consumption/implications.tex <==
In this section, we first briefly summarize the main findings of our RQs. Then, we discuss the implications of those findings in regards to the performance of the just-in-time food recommender systems and their practicality in the just-in-time health interventions.

\begin{itemize}
    \item \textbf{RQ1}: Repeat food consumption is highly ubiquitous, recency biased, and significantly differ across different contexts and demographic groups.
    \item \textbf{RQ2}: Most state-of-the-art recommender systems are not as effective as the best algorithm -- the time-weighted mixture model (\textbf{MixtureTW}), in the just-in-time implicit food recommendation task.
    \item \textbf{RQ3}: The performance of \textbf{MixtureTW} is significantly biased in favor of the users with high repeat consumption tendency, which is manifested in diverse contexts and demographic groups.
\end{itemize}
% \textbf{RQ1:} \textit{What are the overall characteristics of repeat food consumption behavior? Additionally, how do repeat consumption patterns differ across diverse contexts?}
% \begin{itemize}
%   \item Food consumption behaviour involves exploration-exploitation trade-off, with strong recency bias.
%   \item Repeat consumption patterns differed significantly across diverse contexts. Repeat consumption occurs more during breakfasts, weekdays, and for male users and older adults. 
% \end{itemize}
% \textbf{RQ2:} \textit{What is the effectiveness of different state-of-the-art implicit recommender systems in predict daily food consumption patterns of individuals in a just-in-time recommendation setting?}
% \begin{itemize}
%   \item Just-in-time food recommendation task is challenging. Recommender systems which explicitly model the explore-exploit trade-off nature of food choices and the sequential order of consumption outperform the other models.
%   \item Novel food consumption is especially challenging. 
% \end{itemize}
% \textbf{RQ3:} \textit{To what extent does the state-of-the-art food recommender system exhibit algorithmic bias when generating recommendations for diverse groups of users and eating contexts?}
% \begin{itemize}
%   \item Significant algorithmic bias was observed in the context-aware evaluation of MixtureTW.
%   \item User subgroups and eating contexts with higher repeat consumptions benefits more from MixtureTW.
% \end{itemize}

\textbf{Implications for food recommender systems}: To further increase the effectiveness of the just-in-time food recommender systems, several technical improvements can be made. First, additional research should investigate other state-of-the-art temporal models \cite{Kapoor2015}, which may better capture the dynamics of repeat consumptions and the recency bias. Next, the lists of recommended items generated by most algorithms in this study comprise independently selected food items, ignoring the \textit{complementary} nature of food consumption \cite{Teng2012}. Thus, incorporating such item-item complementarity when generating the recommended lists may help improve the performance of the novel items prediction. Lastly, the data preprocessing steps used in this work may not be sufficient in reducing data sparsity in the food consumption data. Therefore, other techniques, such as biclustering, should be further investigated.


% \begin{itemize}
%   \item Recency-bias is from repeat-tendency bias. % Not sure about this point: Repeat consumption is for repeating items consumed recently, thus repeat tendency is from recency?
%   \item Data sparsity. The sparse nature of consumption data restricts the prediction accuracy. Even the best algorithm may not make recommendations readily adoptable for users.
%   \item Item clustering. To improve the effectiveness of recommendation, we may want to group similar items together and make more general recommendations. Instead of recommending 'Low GI Soft Grain Loaf', we can recommend an item cluster, 'Low GI Bread'.
% \end{itemize}

\textbf{Implications for just-in-time interventions}:
Food recommender systems is a potential facilitator of the just-in-time healthy eating interventions where specific food items are adaptively recommended tailored to individuals. The presence of algorithmic bias against the users in certain contexts (e.g., weekends) and demographic groups (e.g., young adults), who are less likely to adopt healthy eating behaviors \cite{Achananuparp2018}, may adversely affect the overall success of the interventions. 
Next, the highly recurring and the recency-biased natures of food consumption emphasize the importance of habit formation \cite{Wood2009} as another facilitator of sustained healthy eating lifestyle. The designs of just-in-time interventions may incorporate both the food recommender systems and the habit formation mechanisms to improve a long-term success of the interventions.
Lastly, the surprising effectiveness of the personal favorite heuristics suggests that a simple rule-based algorithm is a good enough alternative to more sophisticated algorithms (e.g., \textbf{FPMC}, \textbf{HPF}, etc.), especially in the population-scale interventions where computational resources and efficiency are likely ones of the technical constraints.

% [Aek] The paragraph below is relevant:
% Demographic bias
% First, as previously shown, the performance of the best algorithms was biased toward specific demographic groups and eating contexts. Thus, future food recommendation research should focus on improving the prediction accuracy of the underserved groups. More importantly, the best algorithms were not able to effectively predict the daily eating habits of certain demographic groups, who are high-priority targets of behavioral interventions due to their low tendency to adopt healthy eating behaviors \cite{Achananuparp2018}, such as young adults. Similarly, the food consumption patterns in certain eating contexts, where the users are more likely to make unhealthy food choices (e.g., weekends and dinners), were relatively more difficult to predict by the best algorithms. Therefore, food recommender systems should take into account the healthy eating behaviors of the affected groups and contexts when addressing the challenge of algorithmic bias.

% Habit formation and health
% Next, we have shown that a heavy repeat tendency and a strong recency effect in food consumption. This may have implication on user's habit formation. Once the users adopted the food choice recommended, the impact of this single adoption can last long. If the recommendation is a healthier alternative to the previously consumed food, food recommendation may become a key step towards the habit formation of healthy eating.

% Algorithm selection for practical JIT trials
% In addition, for just-in-time intervention, we need to consider computational complexity of the recommender algorithms. In food recommendation trials, recommender systems requiring heavy computational resource (i.e. HPF, FPMC) should be avoided. Personal is a good enough heuristics if no resource at all is available. Statistical models (i.e. Mixture, MixtureTW) is preferred, especially if the repeat consumption propensity and recency bias can be approximated.

% Outline
% \begin{itemize}
%   \item Demographic bias as an indirect effect of recency bias. Algorithm performance is always better for subgroups with higher tendency for repeat consumption. Thus, in general, users with higher repeat consumption will be benefited from the algorithms.
%   \item Habit formation. The heavy repeat consumption and the strong recency effects in food consumption suggest that once the food journalers adopted the healthier food choices recommended, the impact of this single adoption can last long. Thus, food recommendation is a key step towards the habit formation of healthy eating.
%   \item For just-in-time intervention, we need to consider computational complexity. In JIT trials, models requiring heavy computational resource (i.e. HPF, FPMC) should be avoided. Personal is a good enough heuristics if no resource at all is available. Statistical models (i.e. Mixture, MixtureTW) is preferred, especially if the repeat consumption propensity and recency bias can be approximated.
% \end{itemize}


% Old writing
% In the analysis of RQ3, we identify a consistent algorithmic bias across different demographic groups and eating contexts, whereas the recommendation for the user groups / eating context with heavier repeat consumption over novel consumption is always more accurate. 
% Thus, future food recommendation research should focus on improving the prediction accuracy of the underserved groups. More importantly, the best algorithms were not able to effectively predict the daily eating habits of certain demographic groups, who are high-priority targets of behavioral interventions due to their low tendency to adopt healthy eating behaviors \cite{Achananuparp2018}, such as young adults.
% The outcomes of the context-aware evaluation provide important implications for the effectiveness of food recommender systems in the just-in-time healthy eating interventions.Thus, future food recommendation research should focus on improving the prediction accuracy of the underserved groups. More importantly, the best algorithms were not able to effectively predict the daily eating habits of certain demographic groups, who are high-priority targets of behavioral interventions due to their low tendency to adopt healthy eating behaviors \cite{Achananuparp2018}, such as young adults. Similarly, the food consumption patterns in certain eating contexts, where the users are more likely to make unhealthy food choices (e.g., weekends and dinners), were relatively more difficult to predict by the best algorithms. Therefore, food recommender systems should take into account the healthy eating behaviors of the affected groups and contexts when addressing the challenge of algorithmic bias.


% link from RQ1 to RQ2 and 3
% From the analysis of RQ1, we found that food is often repeatedly consumed by food journalers, and recency plays an important role. These imply that food recommendation systems, which consider the explore-exploit trade-off nature of food choices and the sequential order of consumption, may be able to better predict food consumption. Next, we found that the repeat consumption patterns differ by meal occasions, temporal lifestyle factors and demographic groups. This implies that user groups and eating context with heavier repeat consumption over novel consumption can be more accurately predicted by recommender systems. The above implications are consistent with the findings in the RQ2 and RQ3.


==> [DPH 2019] Repeat Food Consumption/intro.tex <==
% Describe problems, motivations, and research gaps
% Describe our focus. How do we specifically address the gaps?
Habitual consumption of balanced and healthful diets is known to positively correlate with long-term physical well-being of individuals \cite{Achananuparp2018}. Yet, a vast number of people, including members of online weight-loss community \cite{Achananuparp2018}, did not tend to eat as healthy as they should on a daily basis. 
Personalized digital health interventions could play a crucial role in helping individuals develop and maintain healthy eating habits.
% The lapse in forming healthy eating habits may play a role in the rising obesity epidemic worldwide.
The emerging paradigm of just-in-time health interventions \cite{Spruijt2014} requires computational models capable of adapting to varying needs of individuals and changing context. Due to their ability to computationally model user preference from past data, food recommender systems can serve as an effective facilitator of the just-in-time healthy eating interventions through the personalized recommendation of healthy food items which are tailored to the individuals' tastes and dietary preferences \cite{Freyne2010,Trattner2017}.

In this study, we identify three main research gaps in current food recommendation research pertaining to its ability to capture the individuals' day-to-day food consumption patterns, which is crucial to its effectiveness in the just-in-time interventions. 
% Gap 1: Repeat consumption was not often considered in recommendation systems.

Firstly, existing food recommender systems have been largely focused on the \textit{utility} or the \textit{novelty} aspect of the recommendations, i.e., the effectiveness of the system is often measured by the user satisfaction of new recommended food items, whereas the \textit{repetitiveness} or the \textit{habitual} aspect of food consumption behavior has so far been under-explored. As a creature of habit, many of our consumption behaviors, including food consumption, exhibit both the \textit{novelty-seeking} \cite{Galak2011} and the \textit{repetitive} \cite{Wood2009} characteristics. The dynamics of novel and repeat consumption behaviors has also been modeled as the exploration (novel) and exploitation (repeat) phenomenon \cite{Anderson2014,Kapoor2015,Kotzias2018}. By taking into account this nature of food consumption behavior, the systems can gain a better understanding of the users' eating habits in various contexts and improve the effectiveness of the recommendations. 
% Gap 2: Reliance on user-item ratings data and their availability.

Secondly, the self-report food consumption data as a form of implicit feedback have not been extensively investigated in food recommendation research. Several food recommender models learn the general user preference from the past user-item rating data on cooking recipes \cite{Trattner2017}. However, in the just-in-time health intervention scenario, this form of explicit feedback may be difficult to obtain since they are likely to impose significant burden on the users having to continually evaluate their own satisfaction of a large amount of food items on a daily basis, many of which have been previously consumed. Given the limitations of the current food logging methods, it is important to understand the effectiveness of implicit-feedback food recommender systems where only the past user-item consumption data are available.

% To-do: add another gap in regards to the context-aware evaluation in food recommender systems.
% Aek LOL:)
% - Recommender system research has just begun to study the fairness in recommendation issue \cite{ekstrand18}.
% - Summarize the findings in Ekstrand et al. \cite{ekstrand18}
% - Similarly, algorithmic bias is a potential problem for food recommender systems and just-in-time health interventions. Users of diverse demographic groups and behaviors may not receive the same benefits from the food recommender algorithms due to the uneven distribution of effectiveness across different groups. In the worst case scenario, inaccurate recommendations may negatively affect the users' health.
% - To our knowledge, this issue has remained unexplored in the evaluation of food recommender systems.

Lastly, research in general recommender systems has just begun to study the fairness in recommendation issue \cite{ekstrand18}. Similarly, algorithmic bias is a potential problem for food recommender systems and just-in-time health interventions. Users from diverse demographic backgrounds and behaviors may not receive the same benefits from the food recommender algorithms due to the potential uneven distribution of effectiveness across different groups. In the worst case scenario, inaccurate recommendations may negatively affect the users' long-term health. To our knowledge, this issue has remained unexplored in the evaluation of food recommender systems.

% Addressing comments from reviewers:
% Contributions compared to prev work in terms of demographics (gender recipe, check*) -> true consumption data was used, prev work used recipe data, check findings are similar or different from the papers

Therefore, we aim to address these gaps in prior work in this study. Specifically, we formulate the following research questions (RQs):

% Therefore, in this paper, we address these gaps in prior work examining how food is repeatedly consumed by food journalers in a real-world setting. We aim to investigate the performance of the just-in-time implicit-feedback food recommender systems in predicting both the novel and repeatedly consumed food items for the next consumption session. Specifically, we formulate the following research questions (RQs):

\textbf{RQ1:} \textit{What are the overall characteristics of repeat food consumption behavior?
% How is food repeatedly consumed by food journalers? 
Additionally, how do repeat consumption patterns differ across diverse contexts, such as meal occasions, temporal lifestyle factors, and demographic groups?}

\textbf{RQ2:} \textit{What is the effectiveness of different state-of-the-art implicit recommender systems in predicting daily food consumption patterns of individuals in a just-in-time recommendation setting?}

\textbf{RQ3:} \textit{To what extent does the state-of-the-art food recommender system exhibit an algorithmic bias when generating recommendations for diverse groups of users and eating contexts?}

% \textbf{RQ4:} \textit{Can the algorithmic biases be reduced with balanced class?}

% \textbf{RQ4:} \textit{Are the food choices in  repeat consumption healthier than those in novel consumption?}

% Summarize our contributions
\textbf{Research Contributions}: In pursuing those questions, we made two major research contributions which are summarized as follows. Firstly, we conducted a quantitative study to thoroughly examine the repeat food consumption behavior of individuals across meal occasions, temporal factors, and demographic factors in a large population of nearly 8K MFP users consisting of 2.7M daily food consumption data over 6 months. To our knowledge, no prior studies have examined these types of food consumption behaviors using self-report food consumption data. Findings from the analysis help establish a better understanding of the food consumption behaviors of the heterogeneous groups of users and the impact of their behaviors on the performance of food recommender systems. 

Secondly, we conducted an offline evaluation of many state-of-the-art recommender system algorithms in the just-in-time food recommendation with implicit feedback data. Specifically, we showed that the simple multinomial mixture model with time weighting, proposed in this paper, significantly outperformed most state-of-the-art algorithms. In addition to the aggregate performance, we also performed a context-aware evaluation to examine the algorithmic bias across different demographic groups and eating contexts.

In what follows, we briefly review related work and describe the dataset and the data preprocessing steps used in the study. Next, we present the analysis of repeat food consumption (RQ1) and the just-in-time food recommendation experiment and the results (RQ2). Then, we present the results of the context-aware evaluation (RQ3), summarize the findings, and discuss their implications. Lastly, the limitations of the study and future work are described.


% Aek's outline:
% \begin{itemize}
%     \item The importance of food and health.
%     \item Food choices are multi-factorial. Convenience is probably the major reason for food choices (need citation).
%     \item Failure of most people to eat healthy. Hence, some technological intervention may be helpful to facilitate behavior change.
%     \item Why and how is food recommender system helpful for healthy eating intervention?
%     \item For most people, it is difficult to break away from daily habits . Without understanding a complete habit of individuals, it is likely that they are going to adopt the recommendation.
%     \item Introduction to just-in-time health intervention and its importance. Next introduce the just-in-time food recommendation problem and its application. The latter can be used to facilitate the former in addition to just predicting daily eating habits for general consumption.
%     \item Introduction to the explore and exploit nature of food consumption (maybe linked to convenience and default bias), leading to novel and repeat consumption.
%     \item Research gap: Novel and repeat food consumption behavior \textit{in the wild} has not been quantitatively examined.
% % characterize user repeat consumption
% % meal occasion carry over, demographic factors...
% % comprehensive...
%     \item Research gap: Just-in-time food recommendation with implicit feedback data (in absence of user-item ratings) is still largely under-explored.
% % worth repeating the points, context-aware, subgroups; 
%     \item Research gap: Novel and repeat food consumption behavior has not been studied before in the recommender systems research area.
% % implicit feedback
% \end{itemize}
% Our contributions are summarized as follows: 
% \begin{itemize}
%  \item Quantitative analysis of novel and repeat food consumption behavior.
%  \item Comprehensive evaluation of just-in-time food recommendation models.
% \end{itemize}

==> [DPH 2019] Repeat Food Consumption/related_work.tex <==
% public health related food studies: diet guild-lines
First, we begin by reviewing past research related to computational studies of food consumption behavior, particularly its exploration (novel) versus exploitation (repeat) nature, and their applications in food recommender systems. 
% They can be categorized into the following groups.

% Psychological studies
% Repeat consumption is studied in psychology and consumer behavior research. One aspect is to examine the hedonic aspect of repeat consumption \cite{Marion2000,Galak2011,Garbinsky2014a,Garbinsky2014b}, i.e. past enjoyment leads to future repeat consumption. Another aspect is to look at the habitual aspect of repeat consumption \cite{Khare2006,Wood2009}, i.e., contextual cues lead to automaticity in future repeat consumption.
% According to Wood \& Neal \cite{Wood2009}, 45% of people's behavior is repeated almost daily and in the same context.
% Also in Wood \& Neal: "Through post hoc inferences, people may judge that responses they repeat frequently must be better than alternatives. These inferences, although not part of habit cuing, may reduce deliberative attempts to change habits."

% Two groups:
% Group 1 is about online food consumption studies
% Group 2 is about recommender systems research, in particular, food recommendation

% Group 1
% Using online data to study food consumption behaviors
%\cite{Abbar2015}, \cite{Mejova2016}, \cite{DeChoudhury2017}, \cite{Ofli2017},  \cite{Achananuparp2018}, \cite{Rokicki2018}

\textbf{Studying food consumption using online data}: Past computational studies have demonstrated various public health monitoring applications, especially pertaining to healthy food consumption \cite{Abbar2015,Mejova2016}, through the use of large-scale data from popular online platforms, such as Twitter, Instagram, Allrecipes, and MyFitnessPal. 
% Most notably, Abbar et al. \cite{Abbar2015} found a high correlation between calorie values of food names mentioned in the Twitter posts and state-wide obesity rates. 
Next, recent studies have investigated the healthiness cues uncovered from food images posted by Instagram users \cite{Ofli2017} and online cooking recipes from Allrecipes \cite{Rokicki2018}. Lastly, online food diaries data from MyFitnessPal users have been used to study individuals' dieting \cite{Weber2016,DeChoudhury2017,Gordon2019}, food substitutes extraction \cite{achananuparp2016}, and healthy eating behaviors \cite{Achananuparp2018}. In contrast to the public health monitoring aspect of previous work, our work focuses on predicting food items likely to be consumed in the next consumption session which has a direct application to the just-in-time health interventions.
% Most notable here is the work of \cite{Abbar2015}, acquiring the Twitter data in the United States. They find a high correlation of calorie values of the food names mentioned in the Twitter posts and state-wide obesity rate and further employ the demographic features to build a prediction model of obesity. 
% While some studies infer the eating activities from posts in online social media, the offline food consumption pattern of individuals have not been well-studied.
% [May merge the following with introduction]
% Eating healthy is not an easy task. One reason is from human bias in food healthiness perception \cite{Ofli2017}. Deriving features from food image, cooking recipes and nutrition facts, a simple model proposed in \cite{Rokicki2018} outperforms the human judgment in the estimation of the healthiness of food. Moreover, people usually do not intake healthy food as they should, even those who set goals and regularly log their consumed food on online diary \cite{Achananuparp2018}.

% Summarize our novel contributions with respect to this group

% Group 2
% Repeat & novel recommendation papers
%\cite{Sarma2012}, \cite{Anderson2014}, \cite{Chen2015}, \cite{Kapoor2015a}, \cite{Kapoor2015b}, \cite{Chen2016}, \cite{Benson2016}, \cite{Kotzias2018}, \cite{Lichman2018}, \cite{Bhagat2018}

% Summarize our novel contributions with respect to this group
\textbf{Modeling novel and repeat consumptions:} Novel and repeat consumptions have been studied in psychology and consumer behavior research from either the hedonic aspect \cite{Marion2000,Galak2011} or the habitual aspect \cite{Khare2006,Wood2009} using conventional methodology, such as questionnaires and interviews. Compared to past consumer behavior studies, our work is one of a few computational studies which quantitatively characterized novel and repeat food consumption behaviors using publicly-available online data. Recently, the novel and/or repeat consumption phenomenon has also been studied in data mining and machine learning research. These studies can be divided into two broad categories. 
The first category focuses on predicting novel items for future consumptions from historical observations -- a common task of general recommender systems. Next, the second category of work examines the recurring nature of past events and consumptions from a variety of online and offline domains, e.g., web search logs \cite{Sarma2012}, online media consumptions and geolocation check-ins \cite{Anderson2014,Kapoor2015,Benson2016,Kotzias2018}, and online product purchases \cite{Bhagat2018}. Within this category, several methods have been proposed to capture the exploration-and-exploitation dynamics underlying the consumption behaviors \cite{Anderson2014,Kapoor2015,Benson2016,Kotzias2018}.
% The second category is sequential recommender, which take sequential behavior of the users into account when generating recommendations. Sequential recommender algorithms are mainly based on a Markov chain models \cite{Zimdars2001,Rendle2010} or time-weighted models \cite{Ding2005,Koren2009}.
Compared to the existing work which mainly investigated online consumptions, our study specifically focuses on characterizing and predicting repeat consumptions from self-report \textit{offline} food consumption data. Our experimental setup is similar to that of Kotzias et al. \cite{Kotzias2018}. In particular, we adopted the recommender algorithms used in their experiments as our baselines. In contrast, we further extended their proposed mixture model by decaying count data over time and analyzed the algorithmic performance and biases in a context-aware evaluation.

% Recommender system is an approach to capture the user preference. Apart from the user ratings, whether or not an item is consumed by the user can be viewed as an indirect reflection of user preference (i.e. implicit feedback). 

% Recommender systems focus either on repeat or novel consumptions are often discussed. Repeat consumption is the user behavior that the user consumed items who has tried before \cite{Chen2015,Chen2016,Kapoor2015a}, whereas novel consumption describes the exploration of new items \cite{Kapoor2015b,Benson2016}. As in \cite{Kotzias2018}, they proposed a simple mixture model that balances repeat and novel consumption, showing surprising good performance compared to models based on matrix factorization. We leverage this model to see which tendency in consumption is more important in eating behavior. Another highlight in recommender systems is on the temporal effects since user preference varies across times and be affected by boredom \cite{Sarma2012,Anderson2014,Benson2016}. In \cite{Lichman2018}, they build a Zero-inflated Poisson regression model that captures data sparsity, repeat consumption, and the temporal changes of preference. Being aware the potential impacts of temporal factors, we characterize the recency and the cyclic pattern that is unique in the food consumption.


% Food/recipe recommendation papers
% - Previous studies focus on rating prediction, whereas our study is similar to one-class collaborative filtering and next-basket recommendation
%\cite{Freyne2010}, \cite{Forbes2011}, \cite{Teng2012}, \cite{Harvey2013}, \cite{Lin2014}, \cite{Ge2015}, \cite{Trattner2017}
\textbf{Food recommender systems:} Past food recommendation research primarily aimed to predict user ratings of online cooking recipes from historical user-item rating data \cite{Trattner2017b}. Several general recommendation methods have been applied to this domain, including content-based filtering \cite{Freyne2010,Teng2012}, collaborative filtering via k-nearest neighbors algorithms  \cite{Harvey2013,Trattner2017} and matrix factorization \cite{Forbes2011,Ge2015,Trattner2017}, etc. Unlike the well-explored problem of rating prediction in food recommender systems, our work focuses on a problem of just-in-time implicit-feedback food recommendation. Specifically, we aim to generate the lists of recommended food items containing both repeat and novel items for the next consumption session (i.e., the next day in our study) by learning from the users' consumption history. Our task setup is comparable to next-basket and sequential recommendation \cite{Rendle2010,Wang2015} 
% Remove Zimdars2001 to save space
% \cite{Zimdars2001,Rendle2010,Wang2015}
which explicitly incorporate sequential information and temporal dynamics \cite{Ding2005,Koren2009} of past behavior in the models. To our knowledge, this particular task has not yet been extensively studied in the food recommendation research \cite{Trattner2017b}.

% In our study, we infer a particular user's favorite from the consumption history of whom and all users, as an one-class collaborative filtering problem. Also, we aim to learn the dynamic pattern of users' preferences across each day. In other words, we consider it as a next-basket recommendation question with information derived from implicit feedback.

==> [DPH 2019] Repeat Food Consumption/results.tex <==
Table~\ref{tbl:recc_results} displays the average recall@5, precision@5, and nDCG@5 across all 146 experiment sessions for the eight algorithms. Overall, there is a significant difference in the performance of different algorithms (p \textless 0.01). 
Particularly, the time-weighted mixture model (MixtureTW) significantly outperformed the other algorithms in all metrics (p \textless 0.01), e.g., +74.2\% of NMF in nDCG@5. The mixture model (Mixture) performs the second best. The mean decay factor $\lambda$ for MixtureTW was 0.812 (S.D. = 0.046), suggesting that recently consumed food items play a larger role in determining the near-future consumptions than food items consumed in older time periods. In addition, the superior performance of Mixture in our experiment is consistent with the results from the previous online consumption experiment \cite{Kotzias2018}.
Next, the performance of the personal heuristic (Personal) is virtually identical to Mixture (-1.3\% of Mixture in nDCG@5). The highly repetitive and context-sensitive nature of food consumption may explain why Personal was as effective as Mixture. Specifically, the average mixture weights $\pi_i$ of the mixture model across all sessions was 0.669 (S.D. = 0.045), indicating that the mixture models tended to assign higher importance to the repeat consumption component than the novel consumption component most of the time. Moreover, the near-identical results also show that Mixture was still relatively less effective in predicting novel items than predicting repeat items. 

The sequential recommender model, FPMC, performed worse than MixtureTW, Mixture and Personal. This is due to the heavy repeat consumption involved in food consumption data, whereas FPMC was originally designed for novel item recommendation only.

Amongst the latent-factor models, NMF performed better than HPF and LDA. The relative performance of the latent-factor models in our experiment differs from those reported in the previous studies \cite{Gopalan2015,Kotzias2018}, where HPF and LDA tended to be more effective than NMF in the implicit-feedback recommendation task. This inconsistency could possibly occur due to: (1) the differences in the experiment setup, i.e., just-in-time recommendation vs. general recommendation; and (2) the differences in data characteristics and user behavior, i.e., offline food consumptions vs. online media consumptions. Unsurprisingly, the simple global popularity heuristics is the least effective algorithm. 


\begin{table}[thp]
\centering
\caption{Performance of different algorithms over all sessions and the standard deviations. The best results are in bold.}
\label{tbl:recc_results}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method & recall@5 & precision@5 & nDCG@5 \\
\midrule
Mixture & 0.370 $\pm$ 0.026 & 0.337 $\pm$ 0.035 & 0.446 $\pm$ 0.034 \\
MixtureTW &  \textbf{0.389} $\pm$ 0.029 &  \textbf{0.352} $\pm$ 0.039 &  \textbf{0.465} $\pm$ 0.038 \\
\midrule
FPMC & 0.355 $\pm$ 0.027 & 0.321 $\pm$ 0.034 & 0.414 $\pm$ 0.035 \\
\midrule
NMF      &  0.185 $\pm$ 0.009 &  0.176 $\pm$ 0.014 &  0.267 $\pm$ 0.012 \\
HPF & 0.099 $\pm$ 0.005 & 0.102 $\pm$ 0.010 & 0.143 $\pm$ 0.002 \\
LDA      &  0.071 $\pm$ 0.013 &  0.060 $\pm$ 0.005 &  0.083 $\pm$ 0.009 \\
\midrule
Global   &  0.054 $\pm$ 0.004 &  0.052 $\pm$ 0.004 &  0.073 $\pm$ 0.004 \\
Personal &  0.366 $\pm$ 0.026 &  0.333 $\pm$ 0.035 &  0.440 $\pm$ 0.034 \\
\bottomrule
\end{tabular}
}
\end{table}

% Error in compilation: The error message "\pdfendlink ended up on a different page" is usually due to a hyperlink (perhaps a citation, or a URL, or cross-reference) somewhere in your PDF, that's breaking across two page (i.e. starting near the end of one page and end on the next).


Overall, these results emphasize the challenging nature of the just-in-time food recommendation task and confirm past findings regarding the strong recency bias of habitual consumptions \cite{Anderson2014} and the oversmoothing tendency of matrix factorization algorithms to overestimate the probability of new items \cite{Kotzias2018}.


==> results.tex <==
Table~\ref{tbl:recc_results} displays the average recall@5, precision@5, and nDCG@5 across all 146 experiment sessions for the eight algorithms. Overall, there is a significant difference in the performance of different algorithms (p \textless 0.01). 
Particularly, the time-weighted mixture model (MixtureTW) significantly outperformed the other algorithms in all metrics (p \textless 0.01), e.g., +74.2\% of NMF in nDCG@5. The mixture model (Mixture) performs the second best. The mean decay factor $\lambda$ for MixtureTW was 0.812 (S.D. = 0.046), suggesting that recently consumed food items play a larger role in determining the near-future consumptions than food items consumed in older time periods. In addition, the superior performance of Mixture in our experiment is consistent with the results from the previous online consumption experiment \cite{Kotzias2018}.
Next, the performance of the personal heuristic (Personal) is virtually identical to Mixture (-1.3\% of Mixture in nDCG@5). The highly repetitive and context-sensitive nature of food consumption may explain why Personal was as effective as Mixture. Specifically, the average mixture weights $\pi_i$ of the mixture model across all sessions was 0.669 (S.D. = 0.045), indicating that the mixture models tended to assign higher importance to the repeat consumption component than the novel consumption component most of the time. Moreover, the near-identical results also show that Mixture was still relatively less effective in predicting novel items than predicting repeat items. 

The sequential recommender model, FPMC, performed worse than MixtureTW, Mixture and Personal. This is due to the heavy repeat consumption involved in food consumption data, whereas FPMC was originally designed for novel item recommendation only.

Amongst the latent-factor models, NMF performed better than HPF and LDA. The relative performance of the latent-factor models in our experiment differs from those reported in the previous studies \cite{Gopalan2015,Kotzias2018}, where HPF and LDA tended to be more effective than NMF in the implicit-feedback recommendation task. This inconsistency could possibly occur due to: (1) the differences in the experiment setup, i.e., just-in-time recommendation vs. general recommendation; and (2) the differences in data characteristics and user behavior, i.e., offline food consumptions vs. online media consumptions. Unsurprisingly, the simple global popularity heuristics is the least effective algorithm. 


\begin{table}[thp]
\centering
\caption{Performance of different algorithms over all sessions and the standard deviations. The best results are in bold.}
\label{tbl:recc_results}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method & recall@5 & precision@5 & nDCG@5 \\
\midrule
Mixture & 0.370 $\pm$ 0.026 & 0.337 $\pm$ 0.035 & 0.446 $\pm$ 0.034 \\
MixtureTW &  \textbf{0.389} $\pm$ 0.029 &  \textbf{0.352} $\pm$ 0.039 &  \textbf{0.465} $\pm$ 0.038 \\
\midrule
FPMC & 0.355 $\pm$ 0.027 & 0.321 $\pm$ 0.034 & 0.414 $\pm$ 0.035 \\
\midrule
NMF      &  0.185 $\pm$ 0.009 &  0.176 $\pm$ 0.014 &  0.267 $\pm$ 0.012 \\
HPF & 0.099 $\pm$ 0.005 & 0.102 $\pm$ 0.010 & 0.143 $\pm$ 0.002 \\
LDA      &  0.071 $\pm$ 0.013 &  0.060 $\pm$ 0.005 &  0.083 $\pm$ 0.009 \\
\midrule
Global   &  0.054 $\pm$ 0.004 &  0.052 $\pm$ 0.004 &  0.073 $\pm$ 0.004 \\
Personal &  0.366 $\pm$ 0.026 &  0.333 $\pm$ 0.035 &  0.440 $\pm$ 0.034 \\
\bottomrule
\end{tabular}
}
\end{table}

% Error in compilation: The error message "\pdfendlink ended up on a different page" is usually due to a hyperlink (perhaps a citation, or a URL, or cross-reference) somewhere in your PDF, that's breaking across two page (i.e. starting near the end of one page and end on the next).


Overall, these results emphasize the challenging nature of the just-in-time food recommendation task and confirm past findings regarding the strong recency bias of habitual consumptions \cite{Anderson2014} and the oversmoothing tendency of matrix factorization algorithms to overestimate the probability of new items \cite{Kotzias2018}.

